Numerical Discretization Methods for the Extended Linear Quadratic Control Problem

In this study, we introduce numerical methods for discretizing continuous-time linear-quadratic optimal control problems (LQ-OCPs). The discretization of continuous-time LQ-OCPs is formulated into differential equation systems, and we can obtain the discrete equivalent by solving these systems. We present the ordinary differential equation (ODE), matrix exponential, and a novel step-doubling method for the discretization of LQ-OCPs. Utilizing Euler-Maruyama discretization with a fine step, we reformulate the costs of continuous-time stochastic LQ-OCPs into a quadratic form, and show that the stochastic cost follows the $\chi^2$ distribution. In the numerical experiment, we test and compare the proposed numerical methods. The results ensure that the discrete-time LQ-OCP derived using the proposed numerical methods is equivalent to the original problem.

==> tex/DiscretizationProblems.tex <==
\section{Discretization Problems}
% Linear Quadratic (LQ) problems have an important role in the control and estimation of linear systems. In this section, we introduce the LQ problems governed by deterministic and stochastic systems. We show that 
% these problem can be discretized by a set of classic equations from Van Loan’s paper~\cite{vanLoan1978MatrixExponential}.
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem 1 - Linear ODE}
We first consider a linear ordinary differential equation (ODE) with ZOH input 
\begin{subequations}
\begin{alignat}{3}
    x(t_k) &= x_k \\
    u(t) &= u_k \qquad &&t_k \leq t < t_{k+1} \\
    \dot x_k(t) &= A_c x(t) + B_c u(t) \qquad && t_k \leq t < t_{k+1}
\end{alignat}
\label{eq:linear-ODE}%
\end{subequations}
where $x_k$ is the initial state. System matrices $A_c$ and $B_c$ may be time dependent but we only consider the time-invariant case in this paper. \\
The solution to the linear ODE for $\tau \in [0, T_s]$ can be defined as
\begin{equation}
\begin{split}
    x(\tau) & = e^{A_c \tau}x_k + \int_0^{\tau}e^{A_ct}B_cdt u_k
    \\
    & = A(\tau)x_k + B(\tau)u_k 
\end{split}
\label{eq:solution-to-linear-ODE}
\end{equation}
Equation~\ref{eq:solution-to-linear-ODE} can be extended to a matrix expression 
\begin{equation}
    \begin{bmatrix}
    x(\tau) \\ u(\tau)
    \end{bmatrix} = 
    \begin{bmatrix} A(\tau) & B(\tau) \\ 0 & I \end{bmatrix} 
    \begin{bmatrix} x_k \\ u_k \end{bmatrix} 
\label{eq:xu-matrixform-linear-ODE}
\end{equation}
\begin{proposition}
\label{prop:ODEs-linear-ODE}
The linear ODE system can be solved by following ODEs 
\begin{subequations}
    \begin{alignat}{3}
        \dot A(\tau) &= A_c A(\tau) \qquad && A(0) = I \\
          \dot B(\tau) &= A(\tau) B_c \qquad && B(0) = 0
    \end{alignat}
    \label{eq:ODEs-linear-ODE}%
\end{subequations}
\end{proposition}
%
\begin{proof}
Equation~\ref{eq:ODEs-linear-ODE} comes from the time derivatives of $A(\tau)$ and $B(\tau)$
\begin{subequations}
\begin{align}
    A(\tau)&=e^{A_c \tau} \\
    B(\tau)&=\int_0^{\tau}e^{A_ct}B_cdt
\end{align}
\label{eq:AtBt-linear-ODE}
\end{subequations}
\end{proof}
% These fundamental equations $A(\tau)$ and $B(\tau)$ are the key to discretize the LQ problems. We will next show how $A(\tau)$ and $B{\tau}$ arise in the LQ problems.\\
\begin{proposition}
Consider $\dot{B}(\tau)$ of the proposition~\ref{prop:ODEs-linear-ODE}, an alternative expression is
\begin{equation}
    \dot B(\tau) = A_cB(\tau) + B_c = A(\tau)B_c \qquad  B(0) = 0
\label{eq:alternative-Bt}
\end{equation}
\end{proposition}
This yields another way for solving $B(\tau)$ without computing $A(\tau)$.\\

\begin{proof}
We have 
\begin{equation}
    \begin{split}
        \dot{B}(t) &= A(t) B_c\\
        A_c \dot{B}(t) &= A_c A(t) B_c 
    \end{split}
\end{equation}
Computing the integral for $[0, t]$ we get 
\begin{equation}
    \begin{split}
        A_c \int_0^{\tau} \dot{B}(t) dt &= \int_0^{\tau} \dot{A}(t) dt B_c \\
        A_c \left( B(\tau) - B(0) \right) & = \left(A(\tau) - A(0)\right)B_c
    \end{split}
\end{equation}
because 
\begin{equation}
    A(0) = I \qquad B(0) = 0 \qquad A(\tau)B_c = \dot{B}(\tau) 
\end{equation}
we have 
\begin{equation}
    \begin{split}
        A_c B(\tau) &= A(\tau)B_c - B_c\\
        \dot{B}(\tau) & = A_c B(\tau) + B_c
    \end{split}
\end{equation}
\end{proof}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem II - LQ deterministic}
Let $N \in \mathbb{Z}^{+}$ for $T= NT_s$, the deterministic continuous-time LQ control problem over the N sample intervals is 
\begin{equation}
    \begin{split}
        \phi &= \int_{t_0}^{t_0 + T} l_c(x(t), u(t)) dt \\
        & = \sum_{k=0}^{N-1} I_k(x(t), u(t))dt
    \end{split}
\label{eq:phi-LQ-deterministic}
\end{equation}
The function $I_k(\Tilde{z}(t))$ is 
\begin{equation}
    \begin{split}
        I_k(x(t),u(t)) &= \frac{1}{2} \int_{t_k}^{t_{k+1}} l_c(x(t), u(t)) dt
        \\
        & = \frac{1}{2} \int_{t_k}^{t_{k+1}} \left[x(t) - \bar x(t)\right]' Q_{c,xx} \left[ x(t) - \bar x(t) \right] 
        \\ & \qquad + \left[ u(t) - \bar u(t) \right]' Q_{c,uu} \left[u(t)-\bar u(t) \right] dt
        \\
        & = l_{k,0} + l_{k,1} + l_{k,2}
    \end{split}
\label{eq:vk-LQ-deterministic}
\end{equation}
where
\begin{subequations}
\begin{alignat}{3}
    l_{k,0} &= \frac{1}{2} \int_{t_k}^{k_{k+1}} 
            \begin{bmatrix}
                x(t) \\ u(t)
            \end{bmatrix}' Q_{c,zz}
            \begin{bmatrix}
                x(t) \\ u(t)
            \end{bmatrix} dt
    \\
    l_{k,1} &=  - \int_{t_k}^{k_{k+1}} 
            \left( Q_{c,zz} 
        \begin{bmatrix}
            \bar{x}(t) \\ \bar{u}(t)
        \end{bmatrix}
         \right)'
        \begin{bmatrix}
            x(t) \\ u(t)
        \end{bmatrix} dt
    \\
    l_{k,2} &=  \frac{1}{2}\int_{t_k}^{k_{k+1}} 
                \begin{bmatrix}
                    \bar{x}(t) \\ \bar{u}(t)
                \end{bmatrix}' 
                Q_{c,zz} 
                \begin{bmatrix}
                    \bar{x}(t) \\ \bar{u}(t)
                \end{bmatrix} dt
\end{alignat}
\label{eq:phi1-phi2-phi3-LQ-deterministic}%
\end{subequations}
We consider ZOH condition of $u(t) = u_k$, $\bar{u}(t) = u_k$ and $\bar{x}(t) = x_k$ for $t_k \leq t < t_{k+1}$. In addition, we assume $Q_{c,xx}$ is symmetric and non-negative, $Q_{c,uu}$ is positive definite.\\
\begin{proposition}
\label{prop:ODEs-LQ-deterministic} The deterministic continuous-time LQ problem can be discretized by the following differential equation system 
\begin{subequations}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t) \qquad && A(0) &&= I 
    \\
    \dot B(t) &= A(t) B_c \qquad && B(0) &&= 0
    \\
    \dot Q(t) & = \Gamma(t)' Q_{c,zz} \Gamma(t) \qquad && Q(0) &&= 0
    \\
    \dot M(t) &= - \Gamma(t)' Q_{c,zz}, \qquad &&
    M(0) && = 0
\end{alignat}
\label{eq:ODEs-LQ-deterministic}%
\end{subequations}
where 
\begin{align}
    Q_{c,zz} & = \begin{bmatrix}
        Q_{c,xx} & 0 \\ 0 & Q_{c,uu}
    \end{bmatrix}
    \\
    \Gamma(t) &= \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix} 
\end{align}
The stage cost function of the corresponding discrete-time LQ control problem can be computed as 
\begin{equation}
    \begin{split}
        l_k(x_k, u_k) &= I_k(\Tilde{z}(t)) \\    
        & = \frac{1}{2} \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}' 
        Q \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix} + 
        \left( M \begin{bmatrix}
            \bar{x}_k \\ \bar{u}_k
        \end{bmatrix} \right)'\begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix} + \rho_k
        \\
        & = \frac{1}{2} \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}' Q \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix} + 
        q_k'  \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix} + \rho_k
    \end{split}
\end{equation}
with $Q=Q(T_s)$, $M=M(T_s)$.
\end{proposition}

\begin{proof} Replacing $[x(t); u(t)]$ of equations~\ref{eq:phi1-phi2-phi3-LQ-deterministic} by equation~\ref{eq:xu-matrixform-linear-ODE}, we get $l_{k,0}$, 
\begin{equation}
    \begin{split}
        l_{k,0} &= \frac{1}{2} \int_{t_k}^{k_{k+1}} 
            \begin{bmatrix}
                x(t) \\ u(t)
            \end{bmatrix}' Q_{c,zz}
            \begin{bmatrix}
                x(t) \\ u(t)
            \end{bmatrix} dt
            \\
            & = \frac{1}{2}  \begin{bmatrix} x_k \\ u_k \end{bmatrix}' \int_0^{T_s} 
            \Gamma(t)'
            Q_{c,zz}
            \Gamma(t) dt
            \begin{bmatrix} x_k \\ u_k \end{bmatrix}
            \\
            & = \frac{1}{2}  \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q(T_s) \begin{bmatrix} x_k \\ u_k \end{bmatrix}
    \end{split}
\label{eq:lk0-LQ-deterministic}
\end{equation}
and $l_{k,1}$ becomes
\begin{equation}
    \begin{split}
        l_{k,1} &= - \int_{t_k}^{k_{k+1}} 
            \left( Q_{c,zz} 
        \begin{bmatrix}
            \bar{x}(t) \\ \bar{u}(t)
        \end{bmatrix}
         \right)'
        \begin{bmatrix}
            x(t) \\ u(t)
        \end{bmatrix} dt
        \\
        & = \left( \int_{0}^{T_s} -\Gamma(t)' Q_{c,zz} dt \begin{bmatrix}
            \bar{x}_k \\ \bar{u}_k \end{bmatrix} \right)'  \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}
        \\
        & =  \left( M(T_s) \begin{bmatrix}
            \bar{x}_k \\ \bar{u}_k \end{bmatrix} \right)'  \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}
        \\
        & = q_k' \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}
    \end{split}
\label{eq:lk1-LQ-deterministic}
\end{equation}
and $l_{k,2}$ is 
\begin{equation}
    l_{k,2} = \frac{1}{2} \int_{t_k}^{k_{k+1}} 
            \begin{bmatrix}
                \bar{x}_k \\ \bar{u}_k
            \end{bmatrix}' 
            Q_{c,zz} 
            \begin{bmatrix}
                \bar{x}_k \\ \bar{u}_k
            \end{bmatrix} dt = \rho_k
\label{eq:lk2-LQ-deterministic}
\end{equation}
Consequently, the continuous-time LQ problem can be discretized as 
\begin{equation}
    \begin{split}
        I_{k}(x(t), u(t)) &= l_{k,0} + l_{k,1} + l_{k,2} \\
        & = \frac{1}{2}  \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} x_k \\ u_k \end{bmatrix} +  q_k' \begin{bmatrix}
            x_k \\ u_k
        \end{bmatrix}  + \rho_k
        \\
        & = l_{k}(x_k, u_k)
    \end{split}
\end{equation}
% where the quadratic term matrix $Q$ and the linear term matrix $M$ are defined as 
% \begin{equation}
%     Q = \int_0^{T_s} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}' \begin{bmatrix} Q_{c,xx} & Q_{c,xu} \\ Q_{c,xu}' & Q_{c,uu} \end{bmatrix} \begin{bmatrix} A(t) & B(t) \\ 0 & I  \end{bmatrix} dt
% \label{eq:Qt-LQ-deterministic}
% \end{equation}
% \begin{equation}
%     M = \int_0^{T_s} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}' \begin{bmatrix} M_{c,xx} & 0 \\ M_{c,ux} & M_{c,uu} \end{bmatrix} dt
%  \label{eq:Mt-LQ-deterministic}
% \end{equation}
% and the system matrices are 
% \begin{subequations}
% \begin{alignat}{3}
%     Q_{c,xx} &= Q_{c,x} \quad && Q_{c,xu}&& = 0 \quad && Q_{c,uu} && = Q_{c,u} \\
%     M_{c,xx} &= -Q_{c,x} \quad && M_{c,ux}&&= 0 \quad && M_{c,uu}&&= -Q_{c,u}
% \end{alignat}
% \end{subequations}
% The constant term 
% \begin{equation}
%     \rho_k=\frac{1}{2}\bar{x}_k'Q_{c,x} \bar{x}_k + \frac{1}{2}\bar{u}_k'Q_{c,u}\bar{u}_k
% \end{equation}
% is independent of u, it thus has no influence to the solution. We therefore ignore it in this case.\\

% Consequently, the ODEs~\ref{eq:ODEs-LQ-deterministic} in the proposition~\ref{prop:ODEs-LQ-deterministic} are the time derivatives of $A(\tau)$, $B(\tau)$, $Q(\tau)$ and $M(\tau)$.
\end{proof}

\begin{remark}
Define output $z(t) = C_c x(t) + D_c u(t)$ 
\begin{equation}
    \begin{bmatrix}
        z(t) \\ u(t)  
    \end{bmatrix}
    = \begin{bmatrix}
        C_c & D_c \\
         0  &  I 
    \end{bmatrix}
    \begin{bmatrix}
        A(\tau) & B(\tau) \\
             0  &  I 
    \end{bmatrix}
    \begin{bmatrix}
        x_k \\ u_k
    \end{bmatrix}
\end{equation}
and the stage cost of the corresponding continuous-time LQ problem is 
\begin{equation}
    \begin{split}
        \Tilde{l}_c(z(t),u(t)) &= \frac{1}{2}\left[ z(t) - \bar{z}(t) \right]' \Tilde{Q}_{c,zz} \left[ z(t) - \bar{z}(t) \right] 
        \\ 
        & \quad + \frac{1}{2}\left[ u(t) - \bar{u}(t) \right]' \Tilde{Q}_{c,zz} \left[ u(t) - \bar{u}(t) \right]
        \\
        & = \frac{1}{2} 
            \begin{bmatrix}
                z(t) - \bar{z}(t) \\ u(t) - \bar{u}(t)
            \end{bmatrix}' Q_{c,zz}
            \begin{bmatrix}
                z(t) - \bar{z}(t) \\ u(t) - \bar{u}(t)
            \end{bmatrix} 
    \end{split}
\end{equation}
The differential equation systems $\dot{A}(t)$, $\dot{B}(t)$, $\dot{Q}(t)$ and $\dot{M}(t)$ for the above LQ problem are the same as the proposition~\ref{prop:ODEs-LQ-deterministic} but the system matrices become
\begin{align}
    Q_{c,zz} &= 
    \begin{bmatrix}
        \Tilde{Q}_{c,zz} & 0 \\ 0 & \Tilde{Q}_{c,uu}
    \end{bmatrix}
    \\
    \Gamma(t) &= \begin{bmatrix}
        C_c & D_c \\ 0 & I 
    \end{bmatrix}
    \begin{bmatrix}
        A(t) & B(t) \\ 0 & I
    \end{bmatrix}
\end{align}
\end{remark}


% % Consider the reference tracking objective function $\phi_z$ 
% % \begin{equation}
% %     \begin{split}
% %         \phi_z(t) &= \frac{1}{2} \int_{t_0}^{t} \| z(s) - \bar{z}(s) \|^2_{Q_{c,z}} ds \\
% %         & = \frac{1}{2} \int_{t_0}^{t} \left ( z(s) - \bar{z}(s) \right)' Q_{c,z} \left ( z(s) - \bar{z}(s) \right) ds
% %     \end{split}
% % \label{eq:ref-tracking-LQ-deterministic}
% % \end{equation}
% % and the input regularization objective function $\phi_u$ 
% % \begin{equation}
% %     \begin{split}
% %         \phi_u(t) &= \frac{1}{2} \int_{t_0}^{t} \| u(s) - \bar{u}(s) \|^2_{Q_{c,u}} ds \\
% %         & = \frac{1}{2} \int_{t_0}^{t} \left ( u(s) - \bar{u}(s) \right)' Q_{c,u}  \left ( u(s) - \bar{u}(s) \right) ds 
% %     \end{split}
% % \label{eq:input-regular-LQ-deterministic}
% % % \end{equation}
% % Define a deterministic LQ problem $l_k(x_k, u_k)$ contains the above objective functions
% % \begin{equation}
% %     \begin{split}
% %         l_k(x_k, u_k) &= \phi_{z, k} + \phi_{u, k} \\
% %         & = \frac{1}{2} \int_{t_k}^{t_{k+1}} \| z(t) - \bar{z}(t) \|^2_{Q_{c,z}} + \| u(t) - \bar{u}(t) \|^2_{Q_{c,u}} dt 
% %     \end{split}
% % \end{equation}
% % and it is governed by the deterministic linear ODE 
% % \begin{equation}
% %     \begin{split}
% %         \dot{x}(t) &= A_c x(t) + B_c u(t) \qquad x(t_k) = x_k \\
% %         z(t) &= C_c x(t) + D_c u(t)
% %     \end{split}
% % \end{equation}

% % \textbf{Remark 3.} 
% % The deterministic LQ problem can be reformulated as 
% % \begin{equation}
% %     \begin{split}
% %         l_k(x_k, u_k) & = \frac{1}{2} \int_{t_k}^{t_{k+1}} \| z(t) - \bar{z}(t) \|^2_{Q_{c,z}} + \| u(t) - \bar{u}(t) \|^2_{Q_{c,u}} dt \\
% %         & = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' \overbrace{\begin{bmatrix} Q_{xx,k} & Q_{xu,k} \\ Q_{ux,k} & Q_{uu,k} \end{bmatrix}}^{=Q_k} \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \overbrace{\begin{bmatrix} q_{x,k} \\ q_{u,k} \end{bmatrix}'}^{=q_k'}  \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \rho_k \\
% %       &
% %       = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \rho_k
% %     \end{split}
% % \label{eq:OneStepLQ-LQ-deterministic}
% % \end{equation}
% % The quadratic term matrix $Q_k$ is defined as 
% % \begin{equation}
% %     Q_k = \int_0^{T_s} \begin{bmatrix} A(s) & B(s) \\ 0 & I \end{bmatrix}' \begin{bmatrix} Q_{c,xx} & Q_{c,xu} \\ Q_{c,ux} & Q_{c,uu} \end{bmatrix} \begin{bmatrix} A(s) & B(s) \\ 0 & I  \end{bmatrix} ds
% % \label{eq:Qk(t)-LQ-deterministic}
% % \end{equation}
% % where 
% \begin{equation}
%     \begin{split}
%         Q_{c,xx} &= C_c'Q_{c,z}C_c, \qquad Q_{c,xu} = C_c' Q_{c,z} D_c, \\
%         Q_{c,ux} &= D_c' Q_{c,z} C_c, \qquad Q_{c,uu}= Q_{c,u} + D_c'Q_{c,z}D_c
%     \end{split}
% \end{equation}
% The linear term vector $q_k$ is defined as 
% \begin{equation}
%     \begin{split}
%         q_k &= M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k \end{bmatrix} 
%     \end{split}
% \label{eq:qk(t)-LQ-deterministic}
% \end{equation}
% where 
% \begin{equation}
%     M_k = \int_0^{T_s} \begin{bmatrix} A(s) & B(s) \\ 0 & I \end{bmatrix}' \begin{bmatrix} q_{c,x} & 0 \\ q_{c,ux} & q_{c,u} \end{bmatrix} ds
% \label{eq:Mk(t)-LQ-deterministic}
% \end{equation}
% \begin{equation}
%     q_{c,x} = -C_c' Q_{c,z}, \quad q_{c,ux} = -D_c' Q_{c,z}, \quad q_{c,u} = -Q_{c,u}
% \end{equation}
% We ignore the constant term $\rho_k$ since it has not influence to the solution of the LQ problem. \\
% \textbf{Remark 4.} The quadratic term matrix $Q_k$ can be described as an ODE
% \begin{equation}
%     \begin{split}
%         \dot{Q_k}(\tau) &= \begin{bmatrix} A(\tau) & B(\tau) \\ 0 & I \end{bmatrix}' \begin{bmatrix} Q_{c,xx} & Q_{c,xu} \\ Q_{c,ux} & Q_{c,uu} \end{bmatrix} \begin{bmatrix} A(\tau) & B(\tau) \\ 0 & I \end{bmatrix} 
%         \\
%         Q_k(0) & = 0 
%     \end{split}
% \label{eq:Qt-LQ-deterministic}
% \end{equation}
% and the linear term matrix $M_k$ can also be expressed as an ODE 
% \begin{equation}
%     \begin{split}
%         \dot{M_k}(\tau) &= \begin{bmatrix} A(\tau) & B(\tau) \\ 0 & I \end{bmatrix}' \begin{bmatrix} q_{c,x} & 0 \\ q_{c,ux} & q_{c,u} \end{bmatrix}
%         \\
%         M_k(0) & = 0 
%     \end{split}
% \label{eq:Mt-LQ-deterministic}
% \end{equation}
% where the $A(\tau)$ and $B(\tau)$ are defined in equation~\ref{eq:A(t)B(t)-linear-ODE}.\\
% \textbf{Remark 5.} In particular, the deterministic LQ problem $l_k(x_k,u_k)$ becomes
% \begin{equation}
%     \begin{split}
%         l_k(x_k, u_k) &= \frac{1}{2} \int_{t_k}^{t_{k+1}} \| x(t) - \bar{x}(t) \|^2_{Q_{c,z}} + \| u(t) - \bar{u}(t) \|^2_{Q_{c,u}}
%         \\
%         & = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} x_k \\ u_k \end{bmatrix}
%     \end{split}
% \end{equation}
% when $C_c = I$, $D_c = \mathbf{0}$ and $x(t) = z(t)$. $\bar{x}(t) = \bar{x}_k$ for $t_k \leq t < t_{k+1}$ indicates the state reference. The quadratic term matrix $Q_{k}$ and the linear term matrix $M_k$ of the above LQ problem are the same as equations~\ref{eq:Qt-LQ-deterministic} and~\ref{eq:Mt-LQ-deterministic}.
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem III - Linear SDE}
Consider a linear stochastic differential equation (SDE)
\begin{equation}
    d\mathbf{x}(t) = \left( A_c \mathbf{x}(t) + B_c u(t) \right) dt + G_c d \mathbf{\omega}(t) \quad d\mathbf{\omega}(t) \sim N(0, I dt)
\label{eq:linear-SDE}
\end{equation}
with 
\begin{equation}
    \begin{split}
        \mathbf{x}(t_k) &= \mathbf{x_k} \qquad  \mathbf{x_k} \sim N(\hat{x}_k, P_k) \\
        u(t) &= u_k \qquad  t_k \leq t < t_{k+1} 
    \end{split}
\end{equation}
where the initial state $\mathbf{x_k}$ is a random variable with the mean $\hat{x}_k$ and the covariance $P_k$.\\
The solution to the linear SDE can be defined as 
\begin{equation}
    \begin{split}
        \mathbf{x}(\tau) & = e^{A_c \tau} \mathbf{x_k} + \int_0^{\tau} e^{A_c t} B_c dt u_k + \int_0^{\tau} e^{A_c t} G_c d\mathbf{\omega}(t)
        \\
        &= A(\tau)\mathbf{x}_k + B(\tau) u_k + \mathbf{w}(\tau) 
    \end{split}
\label{eq:solution-to-linear-SDE}
\end{equation}
where $\mathbf{w}(\tau)$ is a normal process 
\begin{equation}
    w(\tau) = \int_{0}^{\tau} e^{A_c t} Gc d \omega(t)
\label{eq:wt-linear-SDE}
\end{equation}
with zero mean and the covariance $R_{ww}(\tau)$
\begin{equation}
    \begin{split}
        R_{ww}(\tau) &= \text{Cov}\left( w(\tau), w(\tau) \right) \\
        &=\int_0^{\tau} e^{A_c s} G_c \left( e^{A_c s} G_c \right)' ds \\
        & = \int_0^{\tau} A(s) G_c G_c' A(s)' ds
    \end{split}
\label{eq:Rwwt-linear-SDE}
\end{equation}
The linear SDE solution can be extended as 
\begin{equation}
    \begin{bmatrix}
        \mathbf{x}(\tau) \\ u(\tau)
    \end{bmatrix} = \begin{bmatrix} A(\tau) & B(\tau) \\
    0 & I \end{bmatrix} \begin{bmatrix} \mathbf{x}_k \\ u_k  \end{bmatrix} + \begin{bmatrix}
        \mathbf{w}(\tau) \\ 0 
    \end{bmatrix}
\end{equation}
\begin{proposition}
\label{prop:ODEs-linear-SDE}
The linear SDE system can be solved by the following ODEs 
\begin{subequations}
\begin{alignat}{3}
     \dot A(\tau) &= A_c A(\tau) \qquad && A(0) = I \\
     \dot B(\tau) &= A(\tau) B_c \qquad && B(0) = 0 \\
     \dot{R}_{ww}(\tau) &= A(\tau) G_c G_c' A(\tau)' \qquad && R_{ww}(0) =0
\end{alignat}
\label{eq:ODEs-linear-SDE}
\end{subequations}

\end{proposition}
\begin{proof}
The proof for $\dot{A}(\tau)$ and $\dot{B}(\tau)$ has been introduced in the linear ODE case. $\dot{R}_{ww}$ is the time derivative of the covariance matrix $R_{ww}(t)$ 
\end{proof}




%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem IV - LQ stochastic}
We now consider the stochastic LQ control problem governed by the linear SDE. The stochastic LQ problem $l_k(x_k, u_k)$ is random, we thus cannot explicitly define what is the minimal/maximum value of the problem. Here we consider the expectation of the function $\bar{l}_k(x_k, u_k) = l_k(x_k, u_k)$ 
\begin{equation}
    \begin{split}
        \bar{l}_k(x_k, u_k) &= E\left[l_k(x_k, u_k) \right] \\
        &=\frac{1}{2} E \left\{ \int_0^{T_s} \| z(t) - \bar{z}(t) \|^2_{Q_{c,z}} + \| u(t) - \bar{u}(t) \|^2_{Q_{c,u}} dt \right\} 
        \\
        &= E \left\{ \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} x_k \\ u_k \end{bmatrix} \right\} + E\left\{
        \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} x_k \\ u_k \end{bmatrix} \right\}
        \\
        & \qquad + E \left\{ \int_0^{T_s} w(t)'Q_{c,xx}w(t) dt \right\}  
        \\
        & = E \left\{ \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} x_k \\ u_k \end{bmatrix} \right\} + \int_0^{T_s} E \left\{  w(t)'Q_{c,xx}w(t) \right\} dt 
        \\ 
        & \qquad + \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix}
    \end{split}
\label{eq:OneStepLQ-LQ-stochastic}
\end{equation}
where $Q_{c,xx} = C_c'Q_{c,z} C_c$, $Q_k$ and $M_k$ are previously described in the deterministic LQ problem. We remove the constant term from the stochastic LQ problem since it has no influence to the solution. \\
\textbf{Remark 8.} Denote 
\begin{equation}
    l_{k, 1} = \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k  \begin{bmatrix} x_k \\ u_k \end{bmatrix} 
    , \qquad 
    l_{k, 2} = w(t)'Q_{c,xx}w(t) 
\end{equation}
Consider the lemma in Åström's book~\cite[Chap. 8, Lemma 3.3]{Karl1970IntroToStoContTheory} (See Chapter 8. Lemma 3.3) for computing the mean value of a quadratic form of normal stochastic variables,
\begin{equation}
    E \left( x'Sx \right) = m'Sm + \text{Tr}\left( SR \right)
\end{equation}
where x is normal with mean m and covariance R.
We can apply this lemma for solving the expectation of $l_{k,1}$ 
\begin{equation}
    \begin{split}
        E \left[ l_{k, 1} \right] &= E \left \{ \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} x_k \\ u_k \end{bmatrix} \right\}
        \\
        &=\begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix} + \text{Tr}\left( Q_k P_k \right)
    \end{split}
\end{equation}
and the expectation of $l_{k, 2}$
\begin{equation}
    \begin{split}
        E \left[  l_{k, 2} \right] &= E \left\{ w(t)' Q_{c,xx} w(t)  \right\}
        \\
        &= \text{Tr}\left( C_c' R_{ww}(t) C_c\right) 
    \end{split}
\end{equation}
Replace the above results in the stochastic LQ problem, we can obtain
\begin{equation}
    \begin{split}
        \bar{l}_{k}(x_k, u_k) & = E\left[l_k(x_k, u_k) \right] \\
        &= \frac{1}{2} E\left[ l_{k,1} \right] +  \int_0^{T_s} E\left[ l_{k,2} \right] dt + \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix}
        \\
        &= \frac{1}{2} \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix}' Q_k \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix} + \text{Tr}\left( Q_k P_k \right) + \text{Tr} \left( C_c'R_{ww}(T_s)C_c \right)
        \\
        & \quad + \left( M_k \begin{bmatrix} \bar{z}_k \\ \bar{u}_k  \end{bmatrix} \right)' \begin{bmatrix} \bar{x}_k \\ u_k \end{bmatrix}
    \end{split} 
\end{equation}
We notice that the matrix trace terms $\text{Tr}\left( Q_k P_k \right)$ and $\text{Tr}\left( C_c' R_{ww}(T_s)C_c \right)$ are independent to x and u. Therefore these terms cannot influence the solution of the stochastic LQ control problem. The other terms of the stochastic LQ problem are the same the deterministic LQ problem.
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Summary}
This section describes the linear ODE and linear ODE systems, and the LQ problem governed
Both the linear ODE, the linear SDE, and LQ problems can be described by a set of ODEs $A(\tau)$, $B(\tau)$, $Q(\tau)$ and $M_{\tau}$. This means that classic numerical methods such as Euler method and Runge-Kutta methods can be applied for solving these ODEs. 



% where we describe the continuous-time state space solution matrices $A(\tau)$ and $B(\tau)$ as ODEs. Therefore, numerical discretization schemes such as Euler methods and Runge-Kutta methods can be applied for solving these matrices.\\






==> tex/ExtendedLQ.tex <==
\section{The Extended Linear Quadratic Control Problem}
\label{sec:ExtendedLQRproblem}

In this paper, we consider the extended linear quadratic control problem described by a continuous-time state space model with different problems related to model predictive control. We focus on how to compute the equivalent discrete-time extended linear quadratic control problem by using the proposed numerical discretization methods.\\
We define the extended linear quadratic control problems by the following problem definitions.\\
$Problem~1.$ The continuous-time extended linear quadratic control problem
\begin{subequations}
	\begin{alignat}{5}
		& \min_{x, u} \quad && \phi = \phi_z + \phi_u \\
	    & s.t.  && x(0) = x_0,\\
	    &       && \dot{x}(t) = A_c x(t) + B_c u(t),  \\
	    &       && z(t) = C_c x(t) + D_c u(t), 
	\end{alignat}
\label{eq:continuous-timeLQ}
\end{subequations}
where u(t) $\in \mathbb{R}^{m}$ is the system input, x(t) $\in \mathbb{R}^{n}$ is the system state, and z(t) $\in \mathbb{R}^p$ is the system output. $A_c$, $B_c$, $C_c$ and $D_c$ are time-invariant state space model matrices. \\
$\phi$ is a linear quadratic cost function defined by the reference tracking objective function $\phi_z$ 
\begin{equation}
    \begin{split}
        \phi_z & = \frac{1}{2} \int_0^T \|W_z(t) \left( z(t) - \bar{z}(t) \right)\|^2_2 dt \\
           & = \frac{1}{2} \int_0^T \left(z(t)-\bar{z}(t) \right)^T Q_z(t) \left( z(t)-\bar{z}(t) \right) dt
    \end{split}
\label{eq:continuous-timeReferenceTracking}
\end{equation}
and input regularization objective function $\phi_u$
\begin{equation}
    \begin{split}
        \phi_u & = \frac{1}{2} \int_0^T \| W_u(t) \left(  u(t) - \bar{u}(t) \right) \|^2_2 dt \\
           & = \frac{1}{2} \int_0^T \left(u(t)-\bar{u}(t) \right)^T Q_u(t) \left( u(t)-\bar{u}(t) \right) dt
    \end{split}
\label{eq:continuous-timeInputRegularization}
\end{equation}
where $\bar{z}(t) \in \mathbb{R}^{p}$ and $\bar{u}(t) \in \mathbb{R}^m$ are the output and input targets. $Q_z(t) \in \mathbb{R}^{p \times p}$ and $Q_u(t) \in \mathbb{m \times m}$ represent the reference tracking objective weight and input regularization objective weight, respectively.\\
$Remark~1.$ For ensuring the convexity of the problem \ref{eq:continuous-timeLQ}, we assume 
\begin{align}
    Q_{z}(t) & \succeq 0, \\
    Q_{u}(t) & \succeq 0, 
\end{align}
such that the extended linear quadratic control problem is strictly convex quadratic program.\\
$Remark~2.$ We assume the zero-order hold for the system input
\begin{equation}
    u(t) = u_k, \qquad t_{k} \leq t < t_{k} + T_s, 
    % \begin{split}
    %     u(t) &= u_k, \qquad t_{k} \leq t < t_{k} + T_s, 
    %     % \bar{z}(t) &= \bar{z}_k, \qquad t_{k} \leq t < t_{k} + T_s, \\
    %     % \bar{u}(t) &= \bar{u}_t, \qquad t_{k} \leq t < t_{k} + T_s,
    % \end{split}
\end{equation}
where $T_s$ is the system sampling time. \\
$Problem~2.$ The discrete-time linear quadratic control problem without terminal cost is
\begin{subequations}
	\begin{alignat}{5}
		& \min_{ \{x_{k+1}, u_k\}^{N-1}} \quad && l_k(x_k, u_k) \\
	    & s.t.  && x(0) = x_0,\\
	    &       && x_{k+1} = A x_k + B u_k,  \\
	    &       && z_k = C x_k + D u_k, 
	\end{alignat}
\label{eq:discrete-timeLQ}
\end{subequations}
where $A$, $B$, $C$ and $D$ are discrete-time state space matrices. The stage cost $l_k(x_k, u_k)$ for $N \in \{0,1,\ldots, N-1 \}$ is defined as 
\begin{equation}
    l_k(x_k, u_k) = \frac{1}{2} \sum_{k=0}^{N-1} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' 
		\overbrace{ \begin{bmatrix} Q_{xx,k} & Q_{xu,k} \\ Q_{ux,k} & Q_{uu,k} \end{bmatrix} }^{=Q_k} \begin{bmatrix} x_k \\ u_k \end{bmatrix} 
		+ \overbrace{ \begin{bmatrix} q_{x, k} \\ q_{u, k}\end{bmatrix}}^{=M_k}' \begin{bmatrix} x_k \\ u_k \end{bmatrix} 
\label{eq:discrete-timeStageCost}
\end{equation}
The main problem considered in this paper is how to compute matrices $Q_k$ and $M_k$ for the equivalent discrete-time linear quadratic control problem. 

%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{THE NUMERICAL DISCRETIZATION SCHEMES} 
In this section, we will present the numerical discretization schemes for computing matrices of the discrete-time extended linear quadratic control problem. For the simplicity, we describe three classic numerical discretization methods, explicit Euler, implicit Euler and trapezoidal. 

\subsection{The Solution of the Continuous-time State Space Model}
The analytic solution of the continuous-time state space model described in equation~\ref{eq:continuous-timeLQ} can be defined as 
\begin{equation}
    \begin{split}
        x(t) = e^{A_c t}x_k + 
    \end{split}
\end{equation}




The objective functions $\phi_z$ can be reformulated as 
\begin{align}
    \phi & = \phi_{z,k} + \phi_{u,k} \\
         & = \frac{1}{2} \int_0^{T_s} \| z(t) - \bar{z}(t)\|^2_{Q_z} + \| u(t) - \bar{u}(t) \|^2_{Q_{c,u}} dt \\
         & = \frac{1}{2} \int_0^{T_s} \left( \begin{bmatrix} z(t) - \bar{z}(t) \\ u(t) - \bar{u}(t) \end{bmatrix} \right)' \begin{bmatrix} Q_{c,z} & 0 \\ 0 & Q_{c,u} \end{bmatrix} \begin{bmatrix} z(t) - \bar{z}(t) \\ u(t) - \bar{u}(t) \end{bmatrix} dt \\
         & = \frac{1}{2} \int_0^{T_s} 
\end{align}



==> tex/Introduction.tex <==
\section{Introduction}
The optimal control theory has been investigated over the last decades and has numerous applications in science and engineering fields. A classic application of the optimal control techniques is the moon lander, where the optimal controller considers the objective to bring the spacecraft to the lunar surface with the lowest amount of fuel \cite{DGLuenberger1979IntroToDS}. In many real-time applications, the optimal controller is implemented in digital form on digital control platforms. One method to develop a digital controller is to design a continuous-time optimal control problem and then derive the discrete-time version of it \cite{Hendricks2008LCD}. Therefore, the numerical discretization approach for the optimal control problem is required. 

There are many research focus on the shooting methods for the discretization of the optimal control problem governed by nonlinear systems (see e.g. \cite{Hicks1971ApproximationMF}, \cite{BOCK19841603}, \cite{Bock2000MultipleShooting}). Classic Euler or Runge-Kutta based discretization methods for the optimal control problems are well-discussed in ( Betts (2001) described optimal control algorithms based on explicit Euler and Runge-Kutta integration. Pytlak (1999) presented the discretization based on implicit Runge-Kutta integration.). Papers [] presented Euler discretization schemes for linear quadratic control problems with bang-bang controls. Later Alt (2012) extended the results to a stable implicit Euler based discretization method. 

In this paper, we focus on the numerical discretization approaches for the extended linear quadratic control problem. The extended linear quadratic control problem is particular important for the model predictive control (MPC) problems (see e.g., \cite{John2011FiniteHorizonMPC}, \cite{BAGTERPJORGENSEN2012187}, \cite{john2004MHEstimationAndControl}). By assuming zero-order hold system inputs, we can reformulate the continuous-time linear quadratic control problem. The integration parts of the reformulated continuous-time extended linear quadratic control problem can be considered ordinary differential equations (ODEs). These ODEs can be solved numerically by classic numerical methods, e.g., explicit Euler, implicit Euler and trapezoidal. The proposed discretization schemes can be used for the discretization of the model predictive control problems. The numerical experiments show that the (insert the numerical example result here). 

This paper is organized as follows. Section 2 describes the continuous-time extended linear quadratic problem, and how it arises in the MPC. In section 3 we introduce the numerical discretization schemes for the continuous-time extended linear quadratic problem. For simplicity, we only describe the solutions of the explicit Euler, implicit Euler and trapezoidal. Numerical examples are given in section 4, where we compare the results of the (describe the numerical examples here). The section 5 is the conclusion and future work. 


==> tex/IntroductionDistribution_NoAppedix.tex <==
\section{Introduction}

We describe very briefly the deterministic and stochastic optimal control problems we are interested in and the discretization of these problems. 


\section{Linear-Quadratic Optimal Control Problems}
\label{sec:LinearQuadraticOptimalControlProblems}

\subsection{Deterministic linear-quadratic optimal control problem}
Consider the deterministic linear quadratic optimal control problem (LQ-OCP)
\begin{subequations}

\label{eq:Deterministic:ContinuousTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{x,u,z,\tilde z} &&\phi = \int_{t_0}^{t_0+T} l_c(\tilde z(t)) dt \\
& s.t. && x(t_0) = \hat x_0 \\
& && u(t) = u_k \quad &&t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && \dot x(t) = A_c x(t) + B_c u(t) \, && t_0 \leq t < t_0+T \\
& && z(t) = C_c x(t) + D_c u(t) \, && t_0 \leq t < t_0+T \\
& && \bar z(t) = \bar z_k  &&t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && \tilde z(t) = z(t) - \bar z(t) && t_0 \leq t < t_0+T
\end{alignat}
\end{subequations}
with the stage cost function
\begin{equation}
\begin{split}
    l_c(\tilde z(t)) &= \frac{1}{2} \norm{ W_z \tilde z(t)  }_2^2
    = \frac{1}{2} \tilde z(t) ' Q_{c} \tilde z(t), 
\end{split}
\label{eq:det-stagecost}
\end{equation}
and $Q_{c} = W_z' W_z$.
This problem is in continuous-time with piecewise constant inputs, $u(t) = u_k$ for $t_k \leq t < t_{k+1}$, and target variables, $\bar z(t) = z_k$ for $t_k \leq t < t_{k+1}$. 


\begin{remark}
Note that the case $C_c = \begin{bmatrix} I \\ 0 \end{bmatrix}$, $D_{c} = \begin{bmatrix} 0  \\ I \end{bmatrix}$, $Q_{c} = \begin{bmatrix} Q_{c,xx} & 0 \\ 0 & Q_{c,uu}\end{bmatrix}$, and $\bar{z}(t) = [\bar{x}(t); \, \bar{u}(t)]$ corresponds to
\begin{equation}
\begin{split}
    l_c(\tilde z(t)) &= \frac{1}{2} \left[x(t) - \bar x(t)\right]' Q_{c,xx} \left[ x(t) - \bar x(t) \right] 
    \\ & \qquad + \frac{1}{2} \left[ u(t) - \bar u(t) \right]' Q_{c,uu} \left[u(t)-\bar u(t) \right]
\end{split}
\end{equation}
{\flushright \hfill $\blacksquare$}
\end{remark}

The corresponding discrete-time linear-quadratic optimal control problem is
\begin{subequations}
\label{eq:Deterministic:DiscreteTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{x,u} \quad &&\phi = \sum_{k\in \mathcal{N}} l_k(x_k,u_k)  \\
& s.t. && x_0 = \hat x_0 \\
& && x_{k+1} = A x_k + B u_k \quad && k \in \mathcal{N}
\end{alignat}    
\end{subequations}
with the stage costs
\begin{equation}
    l_k(x_k,u_k) = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} x_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \rho_k
\label{eq:deterministic-stageCost}
\end{equation}
where the coefficient in the affine term is
\begin{equation}
    q_k =  M \bar{z}_k \qquad k \in \mathcal{N} 
\end{equation}
and the constant term is
\begin{equation}
    \rho_k =  \int_{t_k}^{t_{k+1}} l_c(\bar{z}_k) dt = l_c(\bar z_k) T_s, \quad k \in \mathcal{N}
\end{equation}
The key problem that we address in this paper is 1) formulation of differential equation systems that can be used to compute $(A,B,Q,M)$ such that \eqref{eq:Deterministic:DiscreteTime:LinearQuadraticOCP} is equivalent to \eqref{eq:Deterministic:ContinuousTime:LinearQuadraticOCP}, and 2) numerical methods for solving the resulting systems of differential equations.

\begin{proposition}[Discretization of the deterministic LQ-OCP] The system of differential equations
\begin{subequations}
\label{eq:DeterministicLQ:MatrixODEsystem}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t) \qquad && A(0) = I \\
    \dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
    \dot Q(t) &= \Gamma(t)' Q_{c} \Gamma(t) \qquad && Q(0) = 0  \\
    \dot M(t) &= -\Gamma(t)' Q_{c} \qquad && M(0) = 0
\end{alignat}
where
\begin{equation}
    \Gamma(t) = \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}
\end{equation}
\end{subequations}
may be used to compute $(A,B,Q,M)$ as
\begin{subequations}
\begin{align}
    A = A(T_s) \\
    B = B(T_s) \\
    Q = Q(T_s) \\
    M = M(T_s)
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}
%

\subsection{Certainty equivalent LQ control for a stochastic system}
Consider an initial state $x(t_0)$ model by a random variable,
\begin{subequations}
\begin{align}
    {\bs x}(t_0) & \sim N(\hat x_0,P_0) \\
    d{\bs \omega} (t) &\sim N_{iid}(0, I dt) 
\end{align}
The stochastic system can be described as continuous-time linear stochastic differential equations (SDE)
\begin{alignat}{3}
    d {\bs x}(t) &= \left( A_c {\bs x}(t) + B_c u(t) \right) dt + G_c d{\bs \omega}(t) \\
    {\bs z}(t) &= C_c {\bs x}(t) + D_c  u(t) 
\label{eq:linearSDE}
\end{alignat}
% with piecewise constant inputs 
% \begin{equation}
%     u(t) = u_k \qquad t_k \leq t < t_{k+1}
% \end{equation}
\end{subequations}
The corresponding discrete-time stochastic system is 
\begin{subequations}
\begin{alignat}{3}
    {\bs x}_{k+1} &= A {\bs x_k} + B u_k + {\bs w}_k \\
    {\bs z}_k &= C {\bs x_k} +  D u_k
\end{alignat}
where
\begin{align}
    {\bs x}_0 &\sim N(\hat{x}_0,P_0) \\
    {\bs w}_k &\sim N_{iid}(0,R_{ww})
\end{align}
\end{subequations}

\begin{proposition}[Discretization of the linear SDE]
The system of differential equations
\begin{subequations}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t) \qquad && A(0) = I \\
    \dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
    \dot R_{ww} &= \Phi(t) \Phi(t)' \qquad && R_{ww}(0) = 0
\end{alignat}
where 
\begin{equation}
    \Phi(t) = A(t) G_c
\end{equation}
\end{subequations}
may be used to compute ($A$,$B$,$R_{ww}$,$C$,$D$) as
\begin{subequations}
\begin{align}
    A &= A(T_s) \\
    B &= B(T_s) \\
    R_{ww} &= R_{ww}(T_s) \\
    C &= C_c \\
    D &= D_c
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}


\subsection{Stochastic linear-quadratic optimal control problem}
Consider the stochastic linear quadratic optimal control problem 
\begin{subequations}
\begin{alignat}{5}
& \min_{{\bs x},u,{\bs z},{\tilde{\bs z}}}  && \psi = E \set{ \phi = \int_{t_0}^{t_0+T} l_c({\tilde{\bs z}}(t))dt } \\
& s.t. && {\bs x}(t_0) \sim N(\hat x_0, P_0) \\
& && d{\bs \omega}(t) \sim N_{iid}(0,I dt) \\
& && u(t) = u_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && d {\bs x}(t) = (A_c {\bs x}(t) + B_c u(t))dt + G_c d{\bs \omega}(t) \\
& && {\bs z}(t) = C_c {\bs x}(t) + D_c u(t) \\
& && {\bar z}(t) = \bar z_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && {\tilde {\bs z}}(t) = {\bs z}(t) - \bar{z}(t)
\end{alignat}
\label{eq:Cont-Stc-LQ-OCP}
\end{subequations}
The corresponding discrete-time stochastic linear quadratic optimal control problem is 
\begin{subequations}
\begin{alignat}{5}
& \min_{{\bs x},u} \quad && \psi = E\set{\phi = \sum_{k \in \mathcal{N}} l_k({\bs x}_k,u_k)+  l_{s,k} (\bs{x}_k,u_k)}  \\
& s.t. && {\bs x}_0 \sim N(\hat x_0, P_0) \\
& && {\bs w_k} \sim N_{iid}(0,R_{ww}) \qquad \qquad \: k \in \mathcal{N} \\
& && {\bs x}_{k+1} = A {\bs x}_k + B u_k + {\bs w}_k \qquad k \in \mathcal{N} 
\end{alignat}
\end{subequations}
where the stage cost function $l_k(\bs{x}_k, u_k)$ is
\begin{subequations}
    \begin{equation}
    l_k(\bs{x}_k,u_k) = \frac{1}{2} \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + \rho_k
    \end{equation}
and the stochastic stage cost function $l_{s,k}(\bs{x}_k, u_k)$ is
    \begin{equation}
        l_{s,k}(\bs{x}_k, u_k) = \int_{t_k}^{t_{k+1}} \frac{1}{2} \bs{W}(t)' Q_{c,ww} \bs{W}(t) + \bs{q}_{s,k}' \bs{W}(t) dt
    \end{equation}
\end{subequations}
The matrices $Q$, $q_k$ and $\rho_k$ of $l_k(\bs{x}_k, u_k)$ are identical to the deterministic case. The system matrices of $l_{s,k}$ are
\begin{subequations}
    \begin{align}
        \bs{W}(t) &= \int_{0}^{t} A(s) G_c d\omega(s) \\
        Q_{c,ww} &= C_c' Q_{c,zz} C_c \\
        \bs{q}_{s,k} &= C_c' Q_{c,zz} \bs{\Tilde{z}}_k   \\
        \bs{\Tilde{z}}_k &= \Gamma(t) \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} - \bar{z}_k
    \end{align}
\end{subequations}
The expectation of the stochastic linear quadratic optimal control problem is 
\begin{subequations}
\begin{alignat}{5}
& \min_{x,u} \quad && \psi = \sum_{k \in \mathcal{N}} l_k(x_k,u_k) + \frac{1}{2}\text{tr}\left( Q \bar{P}_k \right)\\
& s.t. && x_0 = \hat x_0 \\
& &&  x_{k+1} = A x_k + B u_k \quad && k \in \mathcal{N} 
\end{alignat}
\label{eq:meanOfStochasticCosts}
\end{subequations}
where 
\begin{subequations}
    \begin{equation}
    \begin{bmatrix}
            \bs{x}_k \\ u_k
        \end{bmatrix} \sim N(m_k, \bar{P}_k),
    \quad 
    m_k = \begin{bmatrix}
        x_k \\ u_k
    \end{bmatrix},
    \quad 
    \bar{P}_k = \begin{bmatrix} P_k & 0 \\ 0 & 0 \end{bmatrix}
\end{equation}
    %
\begin{equation}
    P_{k+1} = A P_k A' + R_{ww}
\end{equation}
\end{subequations}



% The mean of the stochastic linear quadratic optimal control problem is 
% \begin{subequations}
% \begin{alignat}{5}
% & \min_{x,u} \quad && \psi = \sum_{k \in \mathcal{N}} l_k(x_k,u_k) + \psi_{tr} \\
% & s.t. && x_0 = \hat x_0 \\
% & &&  x_{k+1} = A x_k + B u_k \quad && k \in \mathcal{N} 
% \end{alignat}
% \end{subequations}
% where 
% \begin{equation}
%     \psi_{tr} = \text{tr}(Q_c (C_c P_0 C_c')) + \int_{t_0}^{t_0+T} \text{tr} \left( Q_c R_{zz}(t) \right) dt
% \end{equation}
\begin{proposition}[Discretization of the stochastic LQ-OCP]
The system of differential equations
\begin{subequations}
\label{eq:StochasticLQG:MatrixODEsystem}
\begin{alignat}{3}
\dot A(t) &= A_c A(t) \qquad && A(0) = I \\
\dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
\dot R_{ww}(t) &= \Phi(t) \Phi(t)' \qquad && R_{ww}(0) = 0 \\
\dot Q(t) &= \Gamma(t)' Q_{c} \Gamma(t)  && Q(0) = 0 \\
\dot M(t) &= -\Gamma(t)' Q_{c} \qquad && M(0) = 0 
% \\ \dot Q_{ww}(t) &= \Lambda(t)' Q_{c,zz} \Lambda(t) \qquad && Q_{ww}(0) = 0 
\end{alignat}
where
\begin{align}
    \Phi(t) &= A(t) G_c \\
    \Gamma(t) &= \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}  
    % \Lambda(t) &= C_c \Phi(t) 
 % R_{zz}(t) &= \Lambda(t) \Lambda(t)' 
\end{align}
\end{subequations}
can be used to compute $(A,B,R_{ww},Q,M)$ as
\begin{subequations}
\begin{align}
    A &= A(T_s) \\
    B &= B(T_s) \\
    R_{ww} &= R_{ww}(T_s) \\
    Q &= Q(T_s) \\
    M &= M(T_s) 
    % Q_{ww} &= Q_{ww}(T_s)
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}

\begin{proposition}[Distribution of the stochastic costs] 

Using Euler-Maruya (E-M) discretization with sub-sampling $\delta t = \frac{T_s}{n}$, the stochastic system can be expressed as
\begin{subequations}
\begin{alignat}{5}
     x_{k,i} &= A_i x_k + B_i u_k + G_i \Delta \bs{w}_{k,i} \quad \Delta \bs{w}_{k,j} \sim N(0, I \delta t)  
    \\
     \begin{bmatrix}
        \bs{x}_k \\ u_k
    \end{bmatrix} &= \overbrace{\begin{bmatrix}
        A^k \\ 0
    \end{bmatrix}}^{\phi_{x,k}} \bs{x}_0 + \overbrace{\begin{bmatrix}
        \Theta_{u,k} \\ I_{u,k}
    \end{bmatrix}}^{\Gamma_{u,k}} U_{\mathcal{N}} + \overbrace{\begin{bmatrix}
        \Theta_{w,k} \\ 0
    \end{bmatrix}}^{\Gamma_{w,k}} \bs{W}_{\mathcal{N}}
\label{eq:EMSystemDiscretization}
\end{alignat}
where $A_i$, $B_i$ and $G_i$ for $i = 1,2,\ldots,n$ are E-M discretization coefficients
\begin{equation}
    A_i = (I+ \delta A_c)^i \qquad \qquad B_i = \sum_{j=1}^i A(i-j) \delta t B_c 
\end{equation}
and
    \begin{alignat}{3}
        % \bs{w}_k &= \bar{G} \Delta \bs{w}_k
        % \\
        G_i &= \begin{bmatrix}
        A_{n-1}G_c & A_{n-2}G_c & \ldots & 0_{n-i}
        \end{bmatrix}
        \\
        % \bs_{w}_{k,i} &= \sum_{j=1}^i A(t_{k}+i \delta t ) G_c \Delta w_{k,j} 
        % \\
        % \bs{w}_k &= \begin{bmatrix}
        % \bs{w}_{k,1}' &\bs{w}_{k,2}' & \ldots & \bs{w}_{k,n}'
        % \end{bmatrix}' 
        % \\
        \Theta_{u,k} &= \begin{bmatrix}
            A^{k-1}B & A^{k-2}B & \ldots & 0_{\mathcal{N}-k}
        \end{bmatrix}
        \\
        \Theta_{w,k} &= \begin{bmatrix}
            A^{k-1}G & A^{k-2}G & \ldots & 0_{\mathcal{N}-k}  
        \end{bmatrix}
    \end{alignat}
\end{subequations}
$\bs{W}_{\mathcal{N}}$ and $U_{\mathcal{N}}$ are the random variable $\bs{w}_k= I_{w,k} \bs{W}_{\mathcal{N}}$ and the input $u_{k}=I_{u,k} U_{\mathcal{N}}$ over the horizon $\mathcal{N}$, 

% The Euler-Maruyama (E-M) discretization of the stochastic system with a fine time step $\delta t = \frac{T_s}{n}$, $t_i=i \delta t$ for $i = 1,\ldots, n$ is 
% \begin{subequations}
%     \begin{equation}
%         x_{k,i} = A_i x_k + B_i u_k + \bs{w}_{k,i} 
%         \qquad k \in \mathcal{N}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     A_i &= (I+\delta A_c)^i                  
%     \\
%     B_i &= \sum_{j=1}^{i} A(j) \delta t B_c
%     \\
%     \bs{w}_{k,i} & = \sum_{j=1}^{i} A_{i-j} G_c \Delta \bs{w}_{k,j}  \quad \Delta \bs{w}_{k,j} \sim N_{iid}(0, I \delta t)  
%     % \\
%     % G_i &= \begin{bmatrix}
%     %     A_{n-1}G_c & A_{n-2}G_c & \ldots & 0_{n-i}
%     % \end{bmatrix}
%     \\
%     \bs{w}_k &= \begin{bmatrix}
%         \bs{w}_{k,1}' &\bs{w}_{k,2}' & \ldots & \bs{w}_{k,n}'
%     \end{bmatrix}' 
% \end{alignat}
% \end{subequations}




The corresponding E-M expression of the stochastic cost function $\phi$ is 
\begin{equation}
    \begin{split}
        \phi &= \sum_{k \in \mathcal{N}} l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k)
        \\
        &= \sum_{k \in \mathcal{N}} \frac{1}{2} \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \bs{x}_k \\ u_k
        \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k
        \end{bmatrix}  + \rho_k
        \\
        &= \frac{1}{2} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix}' Q_{\mathcal{N}} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + q_{\mathcal{N}}' \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + \rho_{\mathcal{N}}
    \end{split}
\end{equation}
where 
\begin{subequations}
    \begin{alignat}{3}
        \Gamma_i &= \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A_i & B_i \\ 0 & I \end{bmatrix}
        \\
        \Tilde{Q}_c &= C_c' \begin{bmatrix} Q_{c,zz}   & Q_{c,zz} & \ldots & Q_{c,zz} \end{bmatrix}
        \\
        q_k &= M\bar{z}_k + \delta t \Tilde{Q}_c \Omega \bs{w}_k 
        \\
        q_{zw} &=  \delta t \Tilde{Q}_c \bar{Z}_k 
        \\
        \rho_k &= \frac{1}{2} \bs{w}_k' \bar{Q}_{c,ww} \bs{w}_k + \bar{q}_{zw}' \bs{w}_k  +\frac{1}{2} \bar{z}_k' (T_s Q_{c}) \bar{z}_k 
    \end{alignat}
and $\Omega$, $\bar{Z}_k$ and $\bar{Q}_{c,ww}$ are block diagonal matrices 
\begin{alignat}{3}
    \Omega &= \text{diag}(\begin{bmatrix} \Gamma_1 & \Gamma_2 & \ldots & \Gamma_n \end{bmatrix}) 
    \\
    \bar{Z}_k & = \text{diag}(\begin{bmatrix} \bar{z}_k & \bar{z}_k & \ldots & \bar{z}_k \end{bmatrix}) 
    \\
    \bar{Q}_{c,ww} & = \delta t \: \text{diag}(\begin{bmatrix}  Q_{c,ww} & Q_{c,ww} & \ldots & Q_{c,ww} \end{bmatrix}) 
\end{alignat}
\end{subequations}

Using Eq. \eqref{eq:EMSystemDiscretization} to place $[x_k;u_k]$, we reformulate the quadratic problem with $Q_{\mathcal{N}}$, $q_{\mathcal{N}}$ and $\rho_{\mathcal{N}}$. The state vector of the reformulated cost function is normally distributed  
\begin{equation}
    \begin{bmatrix}
      \bs{x}_0 \\ \bs{W}_{\mathcal{N}} 
    \end{bmatrix}
    \sim N(\bar{m}, \bar{P}) \quad \bar{m} = \begin{bmatrix}
        x_0 \\ 0
    \end{bmatrix},
    \quad 
    \bar{P} = \begin{bmatrix}
    P_0 & 0 \\ 0 & P_w
  \end{bmatrix}
\end{equation}
where $P_w = \text{diag}(I\delta t ,I \delta t, \ldots, I \delta t)$.

Based on the theory of integrating the normal in the quadratic domain introduced in \cite{Das2021genchi2}, the stochastic cost $\phi$ follows a generalized $\chi^2$ distribution, and its expectation and variance 
\begin{subequations}
    \begin{alignat}{3}
        & E\set{\phi} = \frac{1}{2}\bar{m}'Q_{\mathcal{N}} \bar m + q_{\mathcal{N}}'\bar m + \rho_{\mathcal{N}} + \frac{1}{2}\text{tr}\left( Q_{\mathcal{N}} \bar P\right)
        \label{eq:meanOfStochasticCosts} 
        \\ 
        \begin{split}
        & V\set{\phi} = q_{\mathcal{N}}' \bar P q_{\mathcal{N}} + 2m'Q_{\mathcal{N}} \bar P q_{\mathcal{N}} + \bar{m}'Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar m \\
        & \qquad \qquad + \frac{1}{2}\text{tr}(Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar P) 
        \label{eq:varOfStochasticCosts}
        \end{split}
    \end{alignat}
\end{subequations}


%  where $x_0$ and $W_{\mathcal{N}}$ are normally distributed
% \begin{subequations}
%     \begin{equation}
%         \bs{\epsilon} = 
%         \begin{bmatrix}
%             \bs{x}_0 \\ \bs{W}_{\mathcal{N}}
%         \end{bmatrix}
%         \sim N(\bar{m}, \bar{P})
%     \end{equation}
% \end{subequations}






% \begin{subequations}
%     \begin{equation}
%         \begin{split}
%             \phi_k &= l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k) \\
%                 % &= \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}'
%                 %      Q \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + \rho_k \\
%                 &= \frac{1}{2} \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix}'
%                     \bar{Q} \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix} + \bar{q}_{k}' \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix} + \bar{\rho}_k
%         \end{split}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     \bs{w}_k = \begin{bmatrix} \bs{w}_{k,0}' & \bs{w}_{k,0}' & \ldots & \bs{w}_{k,n}'\end{bmatrix}' 
% \end{alignat}
% \end{subequations}
% The stochastic costs then can be expressed as 

% \begin{subequations}
%     \begin{equation}
%         \begin{split}
%             \phi &= \sum_{k \in \mathcal{N}}l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k) \\
%                 &= \bs{\epsilon}_k' \bar{Q} \bs{\epsilon}_k + \bar{q}_k' \bs{\epsilon}_k + \bar{\rho}_k
%         \end{split}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     \bs{\epsilon}_K &= [] 
% \end{alignat}
% \end{subequations}
% Based on \cite{Das2021genchi2}, it was shown that the quadratic form 

% the stochastic cost function $\phi$ is a generalized $\chi^2$ variable with the mean and variance 









% The mean and variance of the stochastic cost $\phi$ can be expressed as 

% where 
% \begin{subequations}
%     \begin{equation}
%         \bs{\epsilon}_k = \begin{bmatrix}
%             \bs{x}_k \\ u_k
%         \end{bmatrix} \sim N(m_k, P_k),
%     \quad 
%     m_k = \begin{bmatrix}
%         \hat{x}_k \\ u_k
%     \end{bmatrix},
%     \quad 
%     P_k = \begin{bmatrix} P_k & 0 \\ 0 & 0 \end{bmatrix}
%     \end{equation}
% \end{subequations}
% The cost function $\phi$ of stochastic linear quadratic optimal control problems follows the generalized chi-square distribution. 
% see appendix \ref{appjanEM} and \ref{appjanChi2} for details on the matrices and variance equation.

% The expectation of the stochastic cost function $\phi$ is 
% \begin{equation}
%     \begin{split}
%         E\set{\phi} & = E\set{\int_{t_0}^{t_0+T} l_c(\bs{\Tilde{z}}(t)) dt}
%         \\
%         &= E\set{\sum_{k \in \mathcal{N}} l_k(\bs x_k, u_k) + l_{s, k}(\bs x_k, u_k)} 
%         \\
%         & = \sum_{k \in \mathcal{N}} \frac{1}{2} \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix} + \rho_k + \text{tr}(Q \bar{P}_k)
%     \end{split} 
% \end{equation}
% where $\hat{x}_k$ is the mean value of $\bs x_k$. $\bar{P}_k$ is the covariance matrix of $x$ and $u$ 
% \begin{equation}
%     \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} \sim N \left(\begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix}, \bar{P}_k \right) \qquad \bar{P}_k = \begin{bmatrix}
%         P_k & 0 \\ 0 & 0 
%     \end{bmatrix}
% \end{equation}
%  Using the Euler-Maruyama sub-sampling $\delta t$, the variance of the stochastic cost $\phi$ is
%     \begin{equation}
%         \begin{split}
%             V\set{\phi} &= V\set{\int_{t_0}^{t_0+T} l_c(\bs{\Tilde{z}}(t)) dt}
%             \\
%             &= V\set{\sum_{k \in \mathcal{N}} l_k(\bs x_k, u_k) + l_{s, k}(\bs x_k, u_k)} 
%             \\
%             &= V\set{ \frac{1}{2} \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix}' Q_\mathcal{N} \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix} + q_\mathcal{N}'\begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix} +\rho_\mathcal{N}} \\
%             &= q_\mathcal{N}'Pq_\mathcal{N} + 2m'Q_\mathcal{N}Pq_\mathcal{N} + m'Q_\mathcal{N}PQ_\mathcal{N}m \\
%             & \qquad + \frac{1}{2}tr(Q_\mathcal{N}PQ_\mathcal{N}P)\label{eq:varcost}
%         \end{split}
%     \end{equation}
%     where $W_\mathcal{N}$ contain all the sub-sampling stochastics, with
%     \begin{equation}
%         \begin{split}
%             \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix}\in N(m,P), \quad m = \begin{bmatrix} \hat{x}_0 \\ 0 \end{bmatrix},\quad P = \begin{bmatrix} P_0 & 0\\ 0 & I\delta t \end{bmatrix}
%         \end{split}
%     \end{equation}

{\flushright \hfill $\blacksquare$}
\end{proposition}
%  has the same format as \eqref{eq:deterministic-stageCost}, but with the stochastic system state $\bs{x}_k$.
 
%     \begin{equation}
%         q_k = M \bar{z}_k
%     \end{equation}
    
%     \begin{equation}
%         \rho_k = \int_{t_k}^{t_{k+1}} l_c(\bar z_k) dt = l_c(\bar z_k) T_s
%     \end{equation}
% and the stage cost function $l_{s,k}(\bs{x}_k, u_k)$
%     \begin{equation}
%         l_{s,k}(\bs{x}_k, u_k) = \int_{t_k}^{t_{k+1}} \frac{1}{2} \bs{W}(t)' Q_{w} \bs{W}(t) + \bs{q}_{s,k}' \bs{W}(t) dt
%     \end{equation}

%     \begin{equation}
%         \bs{W}(t) = \int_{0}^{t} A(s)G_c d\omega(s) 
%     \end{equation}



==> tex/IntroductionJBJO.tex <==
\section{Introduction}

We describe very briefly the deterministic and stochastic optimal control problems we are interested in and the discretization of these problems. 


\section{Linear-Quadratic Optimal Control Problems}
\label{sec:LinearQuadraticOptimalControlProblems}

\subsection{Deterministic linear-quadratic optimal control problem}
Consider the deterministic linear-quadratic optimal control problem (LQ-OCP)
\begin{subequations}

\label{eq:Deterministic:ContinuousTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{x,u,z,\tilde z} &&\phi = \int_{t_0}^{t_0+T} l_c(\tilde z(t)) dt \\
& s.t. && x(t_0) = \hat x_0, \\
& && u(t) = u_k, \quad &&t_k \leq t < t_{k+1}, \, k \in \mathcal{N}, \\
& && \dot x(t) = A_c x(t) + B_c u(t), \quad && t_0 \leq t < t_0+T, \\
& && z(t) = C_c x(t) + D_c u(t), \, && t_0 \leq t < t_0+T, \\
& && \bar z(t) = \bar z_k,  &&t_k \leq t < t_{k+1}, \, k \in \mathcal{N}, \\
& && \tilde z(t) = z(t) - \bar z(t), && t_0 \leq t < t_0+T,
\end{alignat}
\end{subequations}
with the stage cost function
\begin{equation}
\begin{split}
    l_c(\tilde z(t)) &= \frac{1}{2} \norm{ W_z \tilde z(t)  }_2^2
    = \frac{1}{2} \tilde z(t) ' Q_{c} \tilde z(t), 
\end{split}
\label{eq:det-stagecost}
\end{equation}
and $Q_{c} = W_z' W_z$.
This problem is in continuous-time with piecewise constant inputs, $u(t) = u_k$ for $t_k \leq t < t_{k+1}$, and target variables, $\bar z(t) = \bar{z}_k$ for $t_k \leq t < t_{k+1}$. 


\begin{remark}
Note that the case $C_c = \begin{bmatrix} I \\ 0 \end{bmatrix}$, $D_{c} = \begin{bmatrix} 0  \\ I \end{bmatrix}$, $Q_{c} = \begin{bmatrix} Q_{c,xx} & 0 \\ 0 & Q_{c,uu}\end{bmatrix}$, and $\bar{z}(t) = [\bar{x}(t); \, \bar{u}(t)]$ corresponds to
\begin{equation}
\begin{split}
    l_c(\tilde z(t)) &= \frac{1}{2} \left[x(t) - \bar x(t)\right]' Q_{c,xx} \left[ x(t) - \bar x(t) \right] 
    \\ & \qquad + \frac{1}{2} \left[ u(t) - \bar u(t) \right]' Q_{c,uu} \left[u(t)-\bar u(t) \right]
\end{split}
\end{equation}
{\flushright \hfill $\blacksquare$}
\end{remark}

The corresponding discrete-time LQ-OCP is
\begin{subequations}
\label{eq:Deterministic:DiscreteTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{ \{ u_k,x_{k+1} \}_{k\in \mathcal{N}} } \quad &&\phi = \sum_{k\in \mathcal{N}} l_k(x_k,u_k)  \\
& s.t. && x_0 = \hat x_0, \\
& && x_{k+1} = A x_k + B u_k, \quad && k \in \mathcal{N},
\end{alignat}    
\end{subequations}
with the stage costs
\begin{equation}
    l_k(x_k,u_k) = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} x_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \rho_k
\label{eq:deterministic-stageCost}
\end{equation}
where the coefficient in the affine term is
\begin{equation}
    q_k =  M \bar{z}_k \qquad k \in \mathcal{N} 
\end{equation}
and the constant term is
\begin{equation}
    \rho_k =  \int_{t_k}^{t_{k+1}} l_c(\bar{z}_k) dt = l_c(\bar z_k) T_s, \quad k \in \mathcal{N}
\end{equation}
The key problem that we address in this paper is 1) formulation of differential equation systems that can be used to compute $(A,B,Q,M)$ such that \eqref{eq:Deterministic:DiscreteTime:LinearQuadraticOCP} is equivalent to \eqref{eq:Deterministic:ContinuousTime:LinearQuadraticOCP}, and 2) numerical methods for solving the resulting systems of differential equations.

\begin{proposition}[Discretization of the deterministic LQ-OCP] The system of differential equations
\begin{subequations}
\label{eq:DeterministicLQ:MatrixODEsystem}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t) \qquad && A(0) = I \\
    \dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
    \dot Q(t) &= \Gamma(t)' Q_{c} \Gamma(t) \qquad && Q(0) = 0  \\
    \dot M(t) &= -\Gamma(t)' Q_{c} \qquad && M(0) = 0
\end{alignat}
where
\begin{equation}
    \Gamma(t) = \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}
\end{equation}
\end{subequations}
may be used to compute $(A,B,Q,M)$ as
\begin{subequations}
\begin{align}
    A = A(T_s) \\
    B = B(T_s) \\
    Q = Q(T_s) \\
    M = M(T_s)
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}
%

\subsection{Certainty equivalent LQ control for a stochastic system}
Consider an initial state $x(t_0)$ model by a random variable,
\begin{subequations}
\begin{align}
    {\bs x}(t_0) & \sim N(\hat x_0,P_0) \\
    d{\bs \omega} (t) &\sim N_{iid}(0, I dt) 
\end{align}
The stochastic system can be described as continuous-time linear stochastic differential equations (SDEs)
\begin{alignat}{3}
    d {\bs x}(t) &= \left( A_c {\bs x}(t) + B_c u(t) \right) dt + G_c d{\bs \omega}(t) \\
    {\bs z}(t) &= C_c {\bs x}(t) + D_c  u(t) 
\label{eq:linearSDE}
\end{alignat}
% with piecewise constant inputs 
% \begin{equation}
%     u(t) = u_k \qquad t_k \leq t < t_{k+1}
% \end{equation}
\end{subequations}
The corresponding discrete-time stochastic system is 
\begin{subequations}
\begin{alignat}{3}
    {\bs x}_{k+1} &= A {\bs x_k} + B u_k + {\bs w}_k \\
    {\bs z}_k &= C {\bs x_k} +  D u_k
\end{alignat}
where
\begin{align}
    {\bs x}_0 &\sim N(\hat{x}_0,P_0) \\
    {\bs w}_k &\sim N_{iid}(0,R_{ww})
\end{align}
\end{subequations}

\begin{proposition}[Discretization of the linear SDE]
The system of differential equations
\begin{subequations}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t) \qquad && A(0) = I \\
    \dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
    \dot R_{ww} &= \Phi(t) \Phi(t)' \qquad && R_{ww}(0) = 0
\end{alignat}
where 
\begin{equation}
    \Phi(t) = A(t) G_c
\end{equation}
\end{subequations}
may be used to compute ($A$,$B$,$R_{ww}$,$C$,$D$) as
\begin{subequations}
\begin{align}
    A &= A(T_s) \\
    B &= B(T_s) \\
    R_{ww} &= R_{ww}(T_s) \\
    C &= C_c \\
    D &= D_c
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}


\subsection{Stochastic linear-quadratic optimal control problem}
Consider the stochastic LQ-OCP
\begin{subequations}
\begin{alignat}{5}
& \min_{{\bs x},u,{\bs z},{\tilde{\bs z}}}  && \psi = E \set{ \phi = \int_{t_0}^{t_0+T} l_c({\tilde{\bs z}}(t))dt } \\
& s.t. && {\bs x}(t_0) \sim N(\hat x_0, P_0) \\
& && d{\bs \omega}(t) \sim N_{iid}(0,I dt) \\
& && u(t) = u_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && d {\bs x}(t) = (A_c {\bs x}(t) + B_c u(t))dt + G_c d{\bs \omega}(t) \\
& && {\bs z}(t) = C_c {\bs x}(t) + D_c u(t) \\
& && {\bar z}(t) = \bar z_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N} \\
& && {\tilde {\bs z}}(t) = {\bs z}(t) - \bar{z}(t)
\end{alignat}
\label{eq:Cont-Stc-LQ-OCP}
\end{subequations}
The corresponding discrete-time stochastic LQ-OCP is 
\begin{subequations}
\begin{alignat}{5}
\label{eq:stochasticCostFunction}
& \min_{{\bs x},u} \quad && \psi = E\set{\phi = \sum_{k \in \mathcal{N}} l_k({\bs x}_k,u_k)+  l_{s,k} (\bs{x}_k,u_k)}  \\ 
& s.t. && {\bs x}_0 \sim N(\hat x_0, P_0) \\
& && {\bs w_k} \sim N_{iid}(0,R_{ww}) \qquad \qquad \: k \in \mathcal{N} \\
& && {\bs x}_{k+1} = A {\bs x}_k + B u_k + {\bs w}_k \qquad k \in \mathcal{N} 
\end{alignat}
\end{subequations}
where the stage cost function $l_k(\bs{x}_k, u_k)$ is
\begin{subequations}
    \begin{equation}
    l_k(\bs{x}_k,u_k) = \frac{1}{2} \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + \rho_k
    \end{equation}
and the stochastic stage cost function $l_{s,k}(\bs{x}_k, u_k)$ is
    \begin{equation}
        l_{s,k}(\bs{x}_k, u_k) = \int_{t_k}^{t_{k+1}} \frac{1}{2} \bs{W}(t)' Q_{c,ww} \bs{W}(t) + \bs{q}_{s,k}' \bs{W}(t) dt
    \end{equation}
\end{subequations}
The matrices $Q$, $q_k$ and $\rho_k$ of $l_k(\bs{x}_k, u_k)$ are identical to the deterministic case. The system matrices of $l_{s,k}$ are
\begin{subequations}
    \begin{align}
        \bs{W}(t) &= \int_{0}^{t} A(s) G_c d\omega(s) \\
        Q_{c,ww} &= C_c' Q_{c,zz} C_c \\
        \bs{q}_{s,k} &= \bar{C} Q_{c} \left(\Gamma(t) \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} - \bar{z}_k \right)
    \end{align}
\end{subequations}
The expectation of the stochastic LQ-OCP is 
\begin{subequations}
\begin{alignat}{5}
& \min_{x,u} \quad && \psi = \sum_{k \in \mathcal{N}} l_k(x_k,u_k) + \frac{1}{2}\text{tr}\left( Q \bar{P}_k \right)\\
& s.t. && x_0 = \hat x_0 \\
& &&  x_{k+1} = A x_k + B u_k \quad && k \in \mathcal{N} 
\end{alignat}
\label{eq:meanOfStochasticCosts}
\end{subequations}
where 
\begin{subequations}
    \begin{equation}
    \begin{bmatrix}
            \bs{x}_k \\ u_k
        \end{bmatrix} \sim N(m_k, \bar{P}_k),
    \quad 
    m_k = \begin{bmatrix}
        x_k \\ u_k
    \end{bmatrix},
    \quad 
    \bar{P}_k = \begin{bmatrix} P_k & 0 \\ 0 & 0 \end{bmatrix}
\end{equation}
    %
\begin{equation}
    P_{k+1} = A P_k A' + R_{ww}
\end{equation}
\end{subequations}



% The mean of the stochastic linear quadratic optimal control problem is 
% \begin{subequations}
% \begin{alignat}{5}
% & \min_{x,u} \quad && \psi = \sum_{k \in \mathcal{N}} l_k(x_k,u_k) + \psi_{tr} \\
% & s.t. && x_0 = \hat x_0 \\
% & &&  x_{k+1} = A x_k + B u_k \quad && k \in \mathcal{N} 
% \end{alignat}
% \end{subequations}
% where 
% \begin{equation}
%     \psi_{tr} = \text{tr}(Q_c (C_c P_0 C_c')) + \int_{t_0}^{t_0+T} \text{tr} \left( Q_c R_{zz}(t) \right) dt
% \end{equation}
\begin{proposition}[Discretization of the stochastic LQ-OCP]
The system of differential equations
\begin{subequations}
\label{eq:StochasticLQG:MatrixODEsystem}
\begin{alignat}{3}
\dot A(t) &= A_c A(t) \qquad && A(0) = I \\
\dot B(t) &= A(t) B_c \qquad && B(0) = 0 \\
\dot R_{ww}(t) &= \Phi(t) \Phi(t)' \qquad && R_{ww}(0) = 0 \\
\dot Q(t) &= \Gamma(t)' Q_{c} \Gamma(t)  && Q(0) = 0 \\
\dot M(t) &= -\Gamma(t)' Q_{c} \qquad && M(0) = 0 
% \\ \dot Q_{ww}(t) &= \Lambda(t)' Q_{c,zz} \Lambda(t) \qquad && Q_{ww}(0) = 0 
\end{alignat}
where
\begin{align}
    \Phi(t) &= A(t) G_c \\
    \Gamma(t) &= \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A(t) & B(t) \\ 0 & I \end{bmatrix}  
    % \Lambda(t) &= C_c \Phi(t) 
 % R_{zz}(t) &= \Lambda(t) \Lambda(t)' 
\end{align}
\end{subequations}
can be used to compute $(A,B,R_{ww},Q,M)$ as
\begin{subequations}
\begin{align}
    A &= A(T_s) \\
    B &= B(T_s) \\
    R_{ww} &= R_{ww}(T_s) \\
    Q &= Q(T_s) \\
    M &= M(T_s) 
    % Q_{ww} &= Q_{ww}(T_s)
\end{align}
\end{subequations}
{\flushright \hfill $\blacksquare$}
\end{proposition}


\begin{proposition}[Distribution of the stochastic costs] \label{prop:DistributionofStochasticCost}

Using Euler-Maruyama (EM) discretization, the stochastic costs \eqref{eq:stochasticCostFunction} can be reformulated into isolated stochastic form with deterministic weights $Q_{\mathcal{N}}$, $q_{\mathcal{N}}$ and $\rho_{\mathcal{N}}$,
\begin{subequations}
    \begin{equation}
        \begin{split}
            \phi &= \sum_{k \in \mathcal{N}} l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k)
            \\
            &= \frac{1}{2} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix}' Q_{\mathcal{N}} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + q_{\mathcal{N}}' \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + \rho_{\mathcal{N}}
        \end{split}
    \end{equation}
    \begin{equation}
    \begin{bmatrix}
      \bs{x}_0 \\ \bs{W}_{\mathcal{N}} 
    \end{bmatrix}
    \sim N(\bar{m}, \bar{P}) \quad \bar{m} = \begin{bmatrix}
        x_0 \\ 0
    \end{bmatrix},
    \quad 
    \bar{P} = \begin{bmatrix}
    P_0 & 0 \\ 0 & P_w
  \end{bmatrix}
\end{equation}
\end{subequations}
where $\bs{W}_{\mathcal{N}}$ are sub-sampling random variables over the horizon and its covariance is $P_w = \text{diag}([I\delta t, I\delta t, \ldots, I \delta t])$.

Based on the previous work from \cite{Das2021genchi2}, the reformulated stochastic cost function follows a generalized $\chi^2$ distribution, and its expectation and variance are
\begin{subequations}\label{eq:stochcost}
    \begin{alignat}{3}
        & E\set{\phi} = \frac{1}{2}\bar{m}'Q_{\mathcal{N}} \bar m + q_{\mathcal{N}}'\bar m + \rho_{\mathcal{N}} + \frac{1}{2}\text{tr}\left( Q_{\mathcal{N}} \bar P\right)
        \label{eq:meanOfStochasticCosts} 
        \\ 
        \begin{split}
        & V\set{\phi} = q_{\mathcal{N}}' \bar P q_{\mathcal{N}} + 2m'Q_{\mathcal{N}} \bar P q_{\mathcal{N}} + \bar{m}'Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar m \\
        & \qquad \qquad + \frac{1}{2}\text{tr}(Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar P) 
        \label{eq:varOfStochasticCosts}
        \end{split}
    \end{alignat}
\end{subequations}
The continuous cost follows a generalized $\chi^2$ distribution with mean and variance given by \eqref{eq:stochcost} when taking the limit of the number of integration steps $n \rightarrow \infty$. See appendix \ref{app:DistributionProofs} for details on the distribution of the stochastic cost function.

% The E-M stochastic cost is equivalent to the continuous cost when taking the limit of the number of integration steps $n \rightarrow \infty$. Thus, the stochastic continuous cost follows a generalized $\chi^2$ distribution with mean and variance given by the limit of \eqref{eq:stochcost}. See appendix \ref{app:DistributionProofs} for details on the distribution of the stochastic cost function.
% The Euler-Maruyama (E-M) discretization of the stochastic system with a fine time step $\delta t = \frac{T_s}{n}$, $t_i=i \delta t$ for $i = 1,\ldots, n$ is 
% \begin{subequations}
%     \begin{equation}
%         x_{k,i} = A_i x_k + B_i u_k + \bs{w}_{k,i} 
%         \qquad k \in \mathcal{N}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     A_i &= (I+\delta A_c)^i                  
%     \\
%     B_i &= \sum_{j=1}^{i} A(j) \delta t B_c
%     \\
%     \bs{w}_{k,i} & = \sum_{j=1}^{i} A_{i-j} G_c \Delta \bs{w}_{k,j}  \quad \Delta \bs{w}_{k,j} \sim N_{iid}(0, I \delta t)  
%     % \\
%     % G_i &= \begin{bmatrix}
%     %     A_{n-1}G_c & A_{n-2}G_c & \ldots & 0_{n-i}
%     % \end{bmatrix}
%     \\
%     \bs{w}_k &= \begin{bmatrix}
%         \bs{w}_{k,1}' &\bs{w}_{k,2}' & \ldots & \bs{w}_{k,n}'
%     \end{bmatrix}' 
% \end{alignat}
% \end{subequations}
% The E-M expression of the extended state vector $[x_k; u_k]$ is 
% \begin{subequations}
%     \begin{equation}
%         \begin{bmatrix}
%             \bs{x}_k \\ u_k
%         \end{bmatrix} = \overbrace{\begin{bmatrix}
%             A^k \\ 0
%         \end{bmatrix}}^{\phi_{x,k}} \bs{x}_0 + \overbrace{\begin{bmatrix}
%             \Theta_{u,k} \\ I_{u,k}
%         \end{bmatrix}}^{\Gamma_{u,k}} U_{\mathcal{N}} + \overbrace{\begin{bmatrix}
%             \Theta_{w,k} \\ 0
%         \end{bmatrix}}^{\Gamma_{w,k}} \bs{W}_{\mathcal{N}}
%     \label{eq:EMSystemDiscretization}
%     \end{equation} 
% where $\bs{W}_{\mathcal{N}}$ and $U_{\mathcal{N}}$ are the random variable $\bs{w}_k= I_{w,k} \bs{W}_{\mathcal{N}}$ and the input $u_{k}=I_{u,k} U_{\mathcal{N}}$ over the horizon $\mathcal{N}$, 
%     \begin{alignat}{3}
%         % \bs{w}_k &= \bar{G} \Delta \bs{w}_k
%         % \\
%         % \bar{G} & = \begin{bmatrix} G_1' & G_2' & \ldots & G_{n}' \end{bmatrix}'
%         % \\
%         \Theta_{u,k} &= \begin{bmatrix}
%             A^{k-1}B & A^{k-2}B & \ldots & 0_{\mathcal{N}-k}
%         \end{bmatrix}
%         \\
%         \Theta_{w,k} &= \begin{bmatrix}
%             A^{k-1}G & A^{k-2}G & \ldots & 0_{\mathcal{N}-k}  
%         \end{bmatrix}
%     \end{alignat}
% \end{subequations}
% The corresponding E-M expression of the stochastic cost function $\phi$ is 
% \begin{equation}
%     \begin{split}
%         \phi &= \sum_{k \in \mathcal{N}} l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k)
%         \\
%         &= \sum_{k \in \mathcal{N}} \frac{1}{2} \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \bs{x}_k \\ u_k
%         \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k
%         \end{bmatrix}  + \rho_k
%         \\
%         &= \frac{1}{2} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix}' Q_{\mathcal{N}} \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + q_{\mathcal{N}}' \begin{bmatrix} \bs{x}_0 \\ \bs{W}_{\mathcal{N}} \end{bmatrix} + \rho_{\mathcal{N}}
%     \end{split}
% \end{equation}
% where 
% \begin{subequations}
%     \begin{alignat}{3}
%         \Gamma_i &= \begin{bmatrix} C_c & D_c \end{bmatrix} \begin{bmatrix} A_i & B_i \\ 0 & I \end{bmatrix}
%         \\
%         \Tilde{Q}_c &= C_c' \begin{bmatrix} Q_{c,zz}   & Q_{c,zz} & \ldots & Q_{c,zz} \end{bmatrix}
%         \\
%         q_k &= M\bar{z}_k + \delta t \Tilde{Q}_c \Omega \bs{w}_k 
%         \\
%         q_{zw} &=  \delta t \Tilde{Q}_c \bar{Z}_k 
%         \\
%         \rho_k &= \frac{1}{2} \bs{w}_k' \bar{Q}_{c,ww} \bs{w}_k + \bar{q}_{zw}' \bs{w}_k  +\frac{1}{2} \bar{z}_k' (T_s Q_{c}) \bar{z}_k 
%     \end{alignat}
% and $\Omega$, $\bar{Z}_k$ and $\bar{Q}_{c,ww}$ are block diagonal matrices 
% \begin{alignat}{3}
%     \Omega &= \text{diag}(\begin{bmatrix} \Gamma_1 & \Gamma_2 & \ldots & \Gamma_n \end{bmatrix}) 
%     \\
%     \bar{Z}_k & = \text{diag}(\begin{bmatrix} \bar{z}_k & \bar{z}_k & \ldots & \bar{z}_k \end{bmatrix}) 
%     \\
%     \bar{Q}_{c,ww} & = \delta t \: \text{diag}(\begin{bmatrix}  Q_{c,ww} & Q_{c,ww} & \ldots & Q_{c,ww} \end{bmatrix}) 
% \end{alignat}
% \end{subequations}

% Using Eq. \eqref{eq:EMSystemDiscretization} to place $[x_k;u_k]$, we reformulate the quadratic problem with $Q_{\mathcal{N}}$, $q_{\mathcal{N}}$ and $\rho_{\mathcal{N}}$. The state vector of the reformulated cost function is normally distributed  
% \begin{equation}
%     \begin{bmatrix}
%       \bs{x}_0 \\ \bs{W}_{\mathcal{N}} 
%     \end{bmatrix}
%     \sim N(\bar{m}, \bar{P}) \quad \bar{m} = \begin{bmatrix}
%         x_0 \\ 0
%     \end{bmatrix},
%     \quad 
%     \bar{P} = \begin{bmatrix}
%     P_0 & 0 \\ 0 & P_w
%   \end{bmatrix}
% \end{equation}
% where $P_w = \text{diag}(I\delta t ,I \delta t, \ldots, I \delta t)$.

% Based on the theory of integrating the normal in the quadratic domain introduced in \cite{Das2021genchi2}, the stochastic cost $\phi$ follows a generalized $\chi^2$ distribution, and its expectation and variance 
% \begin{subequations}
%     \begin{alignat}{3}
%         & E\set{\phi} = \frac{1}{2}\bar{m}'Q_{\mathcal{N}} \bar m + q_{\mathcal{N}}'\bar m + \rho_{\mathcal{N}} + \frac{1}{2}\text{tr}\left( Q_{\mathcal{N}} \bar P\right)
%         \label{eq:meanOfStochasticCosts} 
%         \\ 
%         \begin{split}
%         & V\set{\phi} = q_{\mathcal{N}}' \bar P q_{\mathcal{N}} + 2m'Q_{\mathcal{N}} \bar P q_{\mathcal{N}} + \bar{m}'Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar m \\
%         & \qquad \qquad + \frac{1}{2}\text{tr}(Q_{\mathcal{N}} \bar P Q_{\mathcal{N}} \bar P) 
%         \label{eq:varOfStochasticCosts}
%         \end{split}
%     \end{alignat}
% \end{subequations}


%  where $x_0$ and $W_{\mathcal{N}}$ are normally distributed
% \begin{subequations}
%     \begin{equation}
%         \bs{\epsilon} = 
%         \begin{bmatrix}
%             \bs{x}_0 \\ \bs{W}_{\mathcal{N}}
%         \end{bmatrix}
%         \sim N(\bar{m}, \bar{P})
%     \end{equation}
% \end{subequations}






% \begin{subequations}
%     \begin{equation}
%         \begin{split}
%             \phi_k &= l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k) \\
%                 % &= \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}'
%                 %      Q \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + \rho_k \\
%                 &= \frac{1}{2} \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix}'
%                     \bar{Q} \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix} + \bar{q}_{k}' \begin{bmatrix} \bs{x}_0 \\ \bs{w}_k \end{bmatrix} + \bar{\rho}_k
%         \end{split}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     \bs{w}_k = \begin{bmatrix} \bs{w}_{k,0}' & \bs{w}_{k,0}' & \ldots & \bs{w}_{k,n}'\end{bmatrix}' 
% \end{alignat}
% \end{subequations}
% The stochastic costs then can be expressed as 

% \begin{subequations}
%     \begin{equation}
%         \begin{split}
%             \phi &= \sum_{k \in \mathcal{N}}l_k( \bs{x}_k, u_k) +  l_{s,k}(\bs{x}_k, u_k) \\
%                 &= \bs{\epsilon}_k' \bar{Q} \bs{\epsilon}_k + \bar{q}_k' \bs{\epsilon}_k + \bar{\rho}_k
%         \end{split}
%     \end{equation}
% where 
% \begin{alignat}{3}
%     \bs{\epsilon}_K &= [] 
% \end{alignat}
% \end{subequations}
% Based on \cite{Das2021genchi2}, it was shown that the quadratic form 

% the stochastic cost function $\phi$ is a generalized $\chi^2$ variable with the mean and variance 









% The mean and variance of the stochastic cost $\phi$ can be expressed as 

% where 
% \begin{subequations}
%     \begin{equation}
%         \bs{\epsilon}_k = \begin{bmatrix}
%             \bs{x}_k \\ u_k
%         \end{bmatrix} \sim N(m_k, P_k),
%     \quad 
%     m_k = \begin{bmatrix}
%         \hat{x}_k \\ u_k
%     \end{bmatrix},
%     \quad 
%     P_k = \begin{bmatrix} P_k & 0 \\ 0 & 0 \end{bmatrix}
%     \end{equation}
% \end{subequations}
% The cost function $\phi$ of stochastic linear quadratic optimal control problems follows the generalized chi-square distribution. 
% see appendix \ref{appjanEM} and \ref{appjanChi2} for details on the matrices and variance equation.

% The expectation of the stochastic cost function $\phi$ is 
% \begin{equation}
%     \begin{split}
%         E\set{\phi} & = E\set{\int_{t_0}^{t_0+T} l_c(\bs{\Tilde{z}}(t)) dt}
%         \\
%         &= E\set{\sum_{k \in \mathcal{N}} l_k(\bs x_k, u_k) + l_{s, k}(\bs x_k, u_k)} 
%         \\
%         & = \sum_{k \in \mathcal{N}} \frac{1}{2} \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix} + \rho_k + \text{tr}(Q \bar{P}_k)
%     \end{split} 
% \end{equation}
% where $\hat{x}_k$ is the mean value of $\bs x_k$. $\bar{P}_k$ is the covariance matrix of $x$ and $u$ 
% \begin{equation}
%     \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} \sim N \left(\begin{bmatrix} \hat{x}_k \\ u_k \end{bmatrix}, \bar{P}_k \right) \qquad \bar{P}_k = \begin{bmatrix}
%         P_k & 0 \\ 0 & 0 
%     \end{bmatrix}
% \end{equation}
%  Using the Euler-Maruyama sub-sampling $\delta t$, the variance of the stochastic cost $\phi$ is
%     \begin{equation}
%         \begin{split}
%             V\set{\phi} &= V\set{\int_{t_0}^{t_0+T} l_c(\bs{\Tilde{z}}(t)) dt}
%             \\
%             &= V\set{\sum_{k \in \mathcal{N}} l_k(\bs x_k, u_k) + l_{s, k}(\bs x_k, u_k)} 
%             \\
%             &= V\set{ \frac{1}{2} \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix}' Q_\mathcal{N} \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix} + q_\mathcal{N}'\begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix} +\rho_\mathcal{N}} \\
%             &= q_\mathcal{N}'Pq_\mathcal{N} + 2m'Q_\mathcal{N}Pq_\mathcal{N} + m'Q_\mathcal{N}PQ_\mathcal{N}m \\
%             & \qquad + \frac{1}{2}tr(Q_\mathcal{N}PQ_\mathcal{N}P)\label{eq:varcost}
%         \end{split}
%     \end{equation}
%     where $W_\mathcal{N}$ contain all the sub-sampling stochastics, with
%     \begin{equation}
%         \begin{split}
%             \begin{bmatrix} x_k \\ W_\mathcal{N} \end{bmatrix}\in N(m,P), \quad m = \begin{bmatrix} \hat{x}_0 \\ 0 \end{bmatrix},\quad P = \begin{bmatrix} P_0 & 0\\ 0 & I\delta t \end{bmatrix}
%         \end{split}
%     \end{equation}

{\flushright \hfill $\blacksquare$}
\end{proposition}
%  has the same format as \eqref{eq:deterministic-stageCost}, but with the stochastic system state $\bs{x}_k$.
 
%     \begin{equation}
%         q_k = M \bar{z}_k
%     \end{equation}
    
%     \begin{equation}
%         \rho_k = \int_{t_k}^{t_{k+1}} l_c(\bar z_k) dt = l_c(\bar z_k) T_s
%     \end{equation}
% and the stage cost function $l_{s,k}(\bs{x}_k, u_k)$
%     \begin{equation}
%         l_{s,k}(\bs{x}_k, u_k) = \int_{t_k}^{t_{k+1}} \frac{1}{2} \bs{W}(t)' Q_{w} \bs{W}(t) + \bs{q}_{s,k}' \bs{W}(t) dt
%     \end{equation}

%     \begin{equation}
%         \bs{W}(t) = \int_{0}^{t} A(s)G_c d\omega(s) 
%     \end{equation}



==> tex/NumericalMethods.tex <==
\section{Discretization Methods}
In this section, we will discuss differential methods for solving the differential equation system of the continuous-time LQ problems. It is natural to consider algorithms based on numerical integration, such as classic Euler methods and Runge-Kutta methods, since we describe $A(t)$, $B(t)$, $Q(t)$, $M(t)$, and $R_{ww}(t)$ as ODEs. An alternative method for solving the system of differential equations is the matrix exponential method. This method is inspired by the formulas from  Moler~\cite{Moler1978NineteenDubiousWays} and Van Loan~\cite{vanLoan1978MatrixExponential}.
\subsection{Ordinary Differential Equation Methods}
For simplicity, we consider the explicit trapezoidal method with fixed step size for computing the differential equations $A$, $B$, $Q$, $M$ and $R_{ww}$. Define $N \in \mathbb{Z}^{+}$ is the number of steps, $h=\frac{T_s}{N}$ is the step size, and $s=2$ indicates the number of stages. Then we get
\begin{subequations}
    \begin{equation}
        \begin{split}
            A_{k+1} &= A_k + h(\frac{1}{2}\dot{A}_{k,1} + \frac{1}{2}\dot{A}_{k,2})\\
                & = (I+hA_c+\frac{1}{2}h^2A_c^2) A_k \\
                & = \Lambda_k A_k
        \end{split}
        \label{eq:ExplTrapeDiscretizationA(t)}
    \end{equation}
    \begin{equation}
        \begin{split}
            B_{k+1} &= B_k +h(\frac{1}{2}\dot{B}_{k,1} + \frac{1}{2}\dot{B}_{k,2})\\
                &= B_k + (\frac{1}{2}A_{k,1} + \frac{1}{2}A_{k,2}) (hBc) \\
                &= B_k + \Theta_k A_k \bar{B}_c 
        \end{split}
        \label{eq:ExplTrapeDiscretizationB(t)}
    \end{equation}
\end{subequations}
where $A_k = A(kh)$ and $B_k = B(kh)$ for $k \in \set{0, 1, \ldots, N-1}$. $A_{k,i}$ and $B_{k, i}$ for $i \in \set{1,\ldots,s}$ are the stage variables computed from method's Butcher tableau. In this case, we have $A_{k,1} = A_k$, $A_{k,2} = (I+hA_c)A_k$, $B_{k,1} = B_k$ and $B_{k,2}=B_k+hA_{k,1}B_c$. The coefficients for computing the stage variables $A_{k,i}$ are constant for each integration step and only need to be computed once, as long as the step size h is fixed. We can then obtain the stage variable $\dot{B}_{k,i} = A_{k,i} B_c $ from $A_{k,i}$. The system matrices $\Lambda_k$, $\Theta_k$ and $\bar{B}_c$ are defined as 
\begin{equation}
    \Lambda = I+hA_c+\frac{1}{2}h^2A_c^2 \qquad \Theta_k = I+\frac{1}{2}hA_c \qquad \bar{B}_c = hB_c
\label{eq:ExplTrapeDiscretizationLambdaPsiBcbar}
\end{equation}
We observe that the matrix $\Lambda_k$ is constant and only needs to be computed once. Then we can calculate $A_{k+1}$ from $A_{k}$ with one matrix-matrix multiplication. Similarly, the matrix $\Theta_k$ is constant and can be computed offline if we fix the step size. Then we can compute the $B_{k+1}$ from $B_k$ based on \eqref{eq:ExplTrapeDiscretizationB(t)}.\\
In addition, we can extend \eqref{eq:ExplTrapeDiscretizationA(t)} and \eqref{eq:ExplTrapeDiscretizationB(t)} to both explicit and implicit single-step methods. Table~\ref{tab:differentDiscretizationMethods} describes the matrices $\Lambda$ and $\Theta$ for differential equations $A(t)$ and $B(t)$ with explicit and implicit single-step methods. In particular, we must confirm the sub-matrices with inverse in $\Lambda$ and $\Theta$ exist when using implicit methods.
\begin{table}[tb]
    \centering
    \caption{The matrices $\Lambda$ and $\Theta$ with different discretization methods}%
    \label{tab:differentDiscretizationMethods}%
    \begin{tabular}{ p{1.5cm} p{2.9cm}  p{2.9cm}  }
    \hline
    \makecell{Methods} & \makecell{$A_{k+1}=\Lambda_k A_k$ \\ $\Lambda_k$}  & \makecell{$B_{k+1}=B_k + \Theta_k A_k \bar{B}_c$ \\ $\Theta_k$} \\ 
    \hline
    \makecell{Expl. Euler}  &  \makecell{$I+hA_c$}         & \makecell{$I$}   \\
    \makecell{Impl. Euler}  &  \makecell{$(I-hA_c)^{-1}$}  & \makecell{$(I-hA_c)^{-1}$}\\
    \makecell{Expl. Trape.} &  \makecell{$I+hA_c+0.5h^2A_c^2$} & \makecell{$I+0.5hA_c$} \\
    \makecell{Impl. Trape.} &  \makecell{$(I+0.5hA_c)^{-1}(I-$ \\ $0.5hA_c)$} & \makecell{$(I-0.5hA_c)^{-1}$}\\
    \makecell{Expl. RK4} &  \makecell{$I+hA_c+0.5h^2A_c^2+$ \\ $0.1667h^3A_c^3+$ \\$0.0417h^4A_c^4$} & \makecell{$I+0.5hA_c+ 0.1667h^2A_c^2$ \\ $+0.0417h^3A_c^3$}  \\
    \makecell{ESDIRK4}  &  \makecell{$(I-0.4359hA_c)^{-3}(I-$ \\ $0.3076hA_c-$ \\ $0.2377h^2A_c^2)$}  & \makecell{$(I-0.4359hAc)^{-3}(I-$ \\ $0.8076hAc+$ \\ $0.0828h^2Ac^2)$}\\
    \hline
    \end{tabular}
\end{table}
\par
Once we calculate the $A(t)$ and $B(t)$ and their stage variables, the differential equations $R_{ww}$, $Q$ and $M$ can be computed as 
\begin{subequations}
    \begin{equation}
        \begin{split}
        R_{ww,k+1} &= R_{ww,k}+ h(\frac{1}{2} \dot{R}_{ww,k,1} +  \frac{1}{2} \dot{R}_{ww,k,2} ) \\
                  &= R_{ww,k} + \frac{1}{2} A_{k,1} \bar{G}_c A_{k,1}' + \frac{1}{2} A_{k,2} \bar{G}_c A_{k,2}' \\
                  &= R_{ww,k} + \sum_{i=1}^{s} b_i A_{k,i} \bar{G}_c A_{k,i}'
        \end{split}
    \label{eq:ExplTrapeDiscretizationRww(t)}
    \end{equation}
    \begin{equation}
        \begin{split}
        Q_{k+1} &= Q_k + h(\frac{1}{2} \dot{Q}_{k,1} +  \frac{1}{2} \dot{Q}_{k,2} ) \\
                  &= Q_k + \frac{1}{2}\Gamma_{k,1}' \bar{Q}_{c,zz} \Gamma_{k,1}' + \frac{1}{2}\Gamma_{k,2}' \bar{Q}_{c,zz} \Gamma_{k,2}' \\
                  &= Q_k + \sum_{i=1}^{s} b_i \Gamma_{k,i}' \bar{Q}_{c,zz} \Gamma_{k,i}'
        \end{split}
    \label{eq:ExplTrapeDiscretizationQ(t)}
    \end{equation}
    \begin{equation}
        \begin{split}
        M_{k+1} &= M_k + h(\frac{1}{2} \dot{M}_{k,1} +  \frac{1}{2} \dot{M}_{k,2} ) \\
                  &= M_k + \frac{1}{2}\Gamma_{M,1}' \bar{M}_{c,zz} + \frac{1}{2}\Gamma_{k,2}' \bar{M}_{c,zz} \\
                  &= Q_k + \sum_{i=1}^{s} b_i \Gamma_{k,i}' \bar{M}_{c,zz} 
        \end{split}
    \label{eq:ExplTrapeDiscretizationM(t)}
    \end{equation}
\end{subequations}
where $b_i$ for $i \in \set{1, 2, \ldots, s}$ indicates the weights of the method's Butcher tableau. $R_{ww,k,i} = A_{k,i}\bar{G}_c A_{k,i}'$, $Q_{k,i} = \Gamma_{k,i}' \bar{Q}_{c,zz} \Gamma_{k,i}$, $M_{k,i}= \Gamma_{k,i}' \bar{M}_{c,zz}$ are stage variables of $R_{ww}$, $Q$ and $M$, respectively. Both of them can be obtained from $A_{k,i}$ and $B_{k,i}$ with constant coefficients,
\begin{subequations}
    \begin{align}
        \Gamma_{k,i} &= \begin{bmatrix} A_{k,i} & B_{k,i} \\ 0 & I \end{bmatrix}
        \\
        \bar{G}_{c} &= h G_c G_c' 
        \\
        \bar{Q}_{c,zz} &= h \begin{bmatrix} C_C & D_c \end{bmatrix}' Q_{c,zz} \begin{bmatrix} C_C & D_c  \end{bmatrix} 
        \\
        \bar{M}_{c,zz} &= -h \begin{bmatrix} C_C & D_c \end{bmatrix}' Q_{c,zz}
    \end{align}
    \label{eq:Gbar,Gamma_k,Qbar,Mbar}%
\end{subequations}
Consequently, we relate the differential equations $Q$, $M$ and $R_{ww}$ to $A$ and $B$ with constant coefficients. This method takes advantage of the linear, constant coefficients nature of the differential equations system. Therefore, the proposed method is more efficient than the standard Euler and Runge-Kutta methods. Besides, this method avoids solving coupled system equations when using implicit methods, while achieving better stability properties than the explicit methods at the same computational cost.\\
Let us now discuss the possibility of the adaptive step size. The adaptive step size case is less efficient than the fixed step size case, since the coefficient matrices $\Lambda$, $\Theta$, $\bar{Q}_{c,zz}$, $\bar{M}_{c,zz}$ and $\bar{G}_c$ needs to be recompute in each iteration. Besides, the algorithm for adapting step size h also requires more computation. Therefore, the adaptive step size methods cannot take the linear, constant coefficients nature of the differential equations system.
\subsection{Matrix Exponential Method}
Consider a block triangular matrix $C_1$ and it's matrix exponential 
\begin{equation}
    C_1 = \begin{bmatrix} 0 & I & 0 \\ 0 & A_c & B_c \\ 0 & 0 & 0 \end{bmatrix},
    \qquad 
    e^{C_1 t} = 
        \begin{bmatrix}
            \phi_{c_1, 11} & \phi_{c_1, 12} & \phi_{c_1, 13} \\
            0 & \phi_{c_1, 22} & \phi_{c_1, 23}\\
            0 & 0 & \phi_{c_1, 33}
        \end{bmatrix}
\end{equation}
Then $A$, $B$ and $M$ can be expressed as 
\begin{subequations}
    \begin{align}
        A(t) &= e^{A_c t} = \phi_{c_1, 22} \\
        B(t) &= \int_0^t e^{A_c \tau} B_c d\tau = \phi_{c_1, 23} \\
        M(t) &= - \int_0^t \Gamma(t) Q_{c,zz} =  \begin{bmatrix}
                    \phi_{c_1,12} & \phi_{c_1,13}\\
                    0 & I
                \end{bmatrix}' \bar{M}_{c,zz}
    \end{align}
\end{subequations}
where $\bar{M}_{c,zz} = - \begin{bmatrix} C_c & D_c \end{bmatrix}' Q_{c,zz}$ is a constant matrix. $\phi_{c_1, 12}$ and $\phi_{c_1, 13}$ are two integrals
\begin{equation}
    \begin{split}
        \phi_{c_1, 12} = \int_0^t A(\tau) d\tau 
        \qquad 
        \phi_{c_1, 13} = \int_0^t B(\tau) d\tau
    \end{split}
\end{equation}
Define another block triangular matrix $C_2$ and it's matrix exponential 
\begin{subequations}
    \begin{align}
        C_2 & = \begin{bmatrix} -A_c' & I & 0 & 0 \\ 0 & -A_c' & Q_{c,xx} & 0 \\ 0 & 0 & A_c & B_c \\ 0 & 0 & 0 & 0 \end{bmatrix}
        \\
        e^{C_2 t} & = 
        \begin{bmatrix}
            \phi_{c_2, 11} & \phi_{c_2, 12} & \phi_{c_2, 13} & \phi_{c_2, 14} \\
            0 & \phi_{c_2, 22} & \phi_{c_2, 23} & \phi_{c_2, 24}  \\
            0 & 0 & \phi_{c_2, 33} & \phi_{c_2, 34} \\
            0 & 0 & 0 & \phi_{c_2, 44} \\
        \end{bmatrix}
    \end{align}
\end{subequations}
$Q$ can be computed as 
\begin{subequations}
    \begin{align}
        Q_{11}(t) &= A(t)' \phi_{c_2,23}  \\
        Q_{21}(t) &=  Q_{12}(t)' = A(t)' \phi_{c_2,24}' + Q_{c,ux}\phi_{c_1,12} \\
        Q_{22}(t) &= W(t) + Q_{c,ux}\phi_{c_1,13} + \phi_{c_1,13}' \phi_{c,xu}+ tQ_{c,uu} \\
        Q(t) &= \begin{bmatrix} Q_{11}(t) & Q_{12}(t) \\ Q_{21}(t) & Q_{22}(t)  \end{bmatrix}
    \end{align}
\end{subequations}
where 
\begin{subequations}
    \begin{equation}
        \begin{split}
            \bar{Q}_{c,zz} &= \begin{bmatrix} C_C & D_c \end{bmatrix}' Q_{c,zz} \begin{bmatrix} C_C & D_c \end{bmatrix} 
            \\
            & = \begin{bmatrix} Q_{c,xx} & Q_{c,xu} \\ Q_{c,ux} & Q_{c,uu}\end{bmatrix}
        \end{split}
    \end{equation}
    \begin{equation}
        W(t) = \left[ B_c'A(t)'\phi_{c_2,14} \right] + \left[ B_c'A(t)'\phi_{c_2,14} \right]'
    \end{equation}
\end{subequations}
$\phi_{c2, 23}$, $\phi_{c2, 24}$ and $\phi_{c2, 14}$ are three integrals 
\begin{subequations}
    \begin{align}
        \phi_{c_2,23} &= e^{-A_c't} \int_0^t A(\tau)' Q_{c,xx} A(\tau) d\tau \\
        \phi_{c_2,24} &= e^{-A_c't} \int_0^t \int_0^r A(r)' Q_{c,xx} A(\tau)B_c d\tau dr \\
        \phi_{c_2,14} &= e^{-A_c't} \int_0^t \int_0^r \int_0^w A(w)' Q_{c,xx} A(\tau)B_c d\tau dw dr  
    \end{align}
\end{subequations}
For computing $R_{ww}$, we define 
\begin{equation}
    C_3 = 
        \begin{bmatrix} -A_c & G_cG_c' \\ 0 & A_c' \end{bmatrix}
    \qquad 
    e^{C_2 t} = 
        \begin{bmatrix}
            \phi_{c_3, 11} & \phi_{c_3, 12}  \\
            0 & \phi_{c_3, 22} \\
        \end{bmatrix}
\end{equation}
and we get 
\begin{subequations}
    \begin{align}
        \phi_{c_3,12} &= e^{-A_ct} \int_0^t A(\tau) G_c G_c' A(\tau) d\tau
        \\
        R_{ww}(t) &= A(t)' \phi_{c_3,12}
    \end{align}
\end{subequations}
Consequently, we can compute $A(T_s)$, $B(T_s)$, $Q(T_s)$, $M(T_s)$ and $R_{ww}(T_s)$ when $t=T_s$.
% \begin{proposition}
% Consider three triangular matrix $C_1$, $C_2$ and $C_3$
% \begin{subequations}
%     \begin{align}
%         C_1 &= 
%         \begin{bmatrix} 0 & I & 0 \\ 0 & A_c & B_c \\ 0 & 0 & 0 \end{bmatrix}
%         \\
%         C_2 & = 
%         \begin{bmatrix} -A_c' & I & 0 & 0 \\ 0 & -A_c' & Q_{c,xx} & 0 \\ 0 & 0 & A_c & B_c \\ 0 & 0 & 0 & 0 \end{bmatrix}
%         \\
%         C_3 &= 
%         \begin{bmatrix} -A_c & G_cG_c' \\ 0 & A_c' \end{bmatrix}
%     \end{align}
% \end{subequations}
% and their matrix exponential 
% \begin{subequations}
%     \begin{align}
%         e^{C_1 t} &= 
%         \begin{bmatrix}
%             \phi_{c_1, 11} & \phi_{c_1, 12} & \phi_{c_1, 13} \\
%             0 & \phi_{c_1, 22} & \phi_{c_1, 23}\\
%             0 & 0 & \phi_{c_1, 33}
%         \end{bmatrix}
%         \\
%         e^{C_2 t} &= 
%         \begin{bmatrix}
%             \phi_{c_2, 11} & \phi_{c_2, 12} & \phi_{c_2, 13} & \phi_{c_2, 14} \\
%             0 & \phi_{c_2, 22} & \phi_{c_2, 23} & \phi_{c_2, 24}  \\
%             0 & 0 & \phi_{c_2, 33} & \phi_{c_2, 34} \\
%             0 & 0 & 0 & \phi_{c_2, 44} \\
%         \end{bmatrix}
%         \\
%         e^{C_2 t} &= 
%         \begin{bmatrix}
%             \phi_{c_3, 11} & \phi_{c_3, 12}  \\
%             0 & \phi_{c_3, 22} \\
%         \end{bmatrix}
%     \end{align}
% \end{subequations}
% Then the matrices ($A$, $B$, $Q$, $M$, $R_{ww}$) can be computed as 
% \begin{subequations}
%     \begin{align}
%         A(t) &= \phi_{c_1,22} = \phi_{c_2, 33} = \phi_{c_3,22}  \\
%         B(t) &= \phi_{c_1,23} = \phi_{c_2, 34} \\
%         Q_{11}(t) &= \phi_{c_2,33}' \phi_{c_2,23}  \\
%         Q_{12}(t) &= \phi_{c_2,24} \phi_{c_2,33} + \phi_{c_1,12}'Q_{c,xu} \\
%         Q_{21}(t) &= Q_{12}(t)' \\
%         Q_{22}(t) &= K(t) + Q_{c,ux}\phi_{c_1,13} + \phi_{c_1,13}' \phi_{c,xu}\\
%                     & \quad + tQ_{c,uu} \\
%         Q(t) &= \begin{bmatrix} Q_{11}(t) & Q_{12}(t) \\ Q_{21}(t) & Q_{22}(t)  \end{bmatrix}
%         \\
%         M(t) &= \begin{bmatrix}
%                     \phi_{c_1,12} & \phi_{c_1, 13}\\
%                     0 & I 
%                 \end{bmatrix}'
%                 \bar{M}_{c,zz} 
%         \\
%         R_{ww}(t) &= \phi_{c_3,22}' \phi_{c_3,12}
%     \end{align}
% \end{subequations}
% in which 
% \begin{subequations}
%     \begin{align}
%         \phi_{c_1,22} &= \phi_{c_2, 33} = e^{A_c t} \\
%         \phi_{c_1,23} &= \phi_{c_2, 34} = \int_0^t e^{A_c \tau} B_c d\tau \\
%         \phi_{c_1,12} &= \int_0^t A(\tau) d\tau \\
%         \phi_{c_1,13} &= \int_0^t B(\tau) d\tau \\
%         \phi_{c_2,23} &= e^{-A_c't} \int_0^t A(\tau)' Q_{c,xx} A(\tau) d\tau \\
%         \phi_{c_2,24} &= e^{-A_c't} \int_0^t A(\tau)' Q_{c,xx} B(\tau) d\tau \\
%         \phi_{c_2,14} &= e^{-A_c't} \int_0^t A(\tau)' Q_{c,xx} B(\tau) d\tau \\
%         \phi_{c_3,12} &= e^{-A_c t} \int_0^t A(\tau) G_c G_c' A(\tau) d\tau \\
%         K(t) & = \left[ B_c'A(t)'\phi_{c_2,14} \right] + \left[ B_c'A(t)'\phi_{c_2,14} \right]'
%     \end{align}
% \end{subequations}
% \end{proposition}



% \begin{equation}
%     C_1 = 
%     \begin{bmatrix} 
%         0 & I & 0 \\ 
%         0 & A_c & B_c \\
%         0 & 0 & 0 
%     \end{bmatrix}
% \end{equation}
